ODIN: Automated Drift Detection and Recovery in Video Analytics

Recent advances in computer vision have led to a resurgence of interest in visual data analytics. Researchers are developing systems for effectively and efficiently analyzing visual data at scale. A significant challenge that these systems encounter lies in the drift in real-world visual data. For instance, a model for self-driving vehicles that is not trained on images containing snow does not work well when it encounters them in practice. This drift phenomenon limits the accuracy of models employed for visual data analytics. In this paper, we present a visual data analytics system, called ODIN, that automatically detects and recovers from drift. ODIN uses adversarial autoencoders to learn the distribution of high-dimensional images. We present an unsupervised algorithm for detecting drift by comparing the distributions of the given data against that of previously seen data. When ODIN detects drift, it invokes a drift recovery algorithm to deploy specialized models tailored towards the novel data points. These specialized models outperform their non-specialized counterpart on accuracy, performance, and memory footprint. Lastly, we present a model selection algorithm for picking an ensemble of best-fit specialized models to process a given input. We evaluate the efficacy and efficiency of ODIN on high-resolution dashboard camera videos captured under diverse environments from the Berkeley DeepDrive dataset. We demonstrate that ODIN's models deliver 6x higher throughput, 2x higher accuracy, and 6x smaller memory footprint compared to a baseline system without automated drift detection and recovery.

==> Makefile <==
MAIN ?= main
DIFF ?= HEAD^
CODE := $(addsuffix .tex,$(filter-out %.tex,$(wildcard code/*)))
FIGS := $(patsubst %.svg,%.pdf,$(wildcard fig/*.svg))
PLOT := $(patsubst %.gp,%.tex,$(wildcard data/*.gp))
DEPS := rev.tex code/fmt.tex abstract.txt $(CODE) $(FIGS) $(PLOT) 
BTEX := --bibtex-args="-min-crossrefs=99"

all: $(DEPS)
	@TEXINPUTS="sty:" bin/latexrun $(BTEX) $(MAIN)

submit: $(DEPS)
	@for f in $(wildcard submit-*.tex); do \
		TEXINPUTS="sty:" bin/latexrun $$f; \
	done

diff: $(DEPS)
	@bin/diff.sh $(DIFF)

help:
	echo "..."

rev.tex: FORCE
	@printf '\\gdef\\therev{%s}\n\\gdef\\thedate{%s}\n' \
	   "$(shell git rev-parse --short HEAD)"            \
	   "$(shell git log -1 --format='%ci' HEAD)" > $@

code/%.tex: code/%
	pygmentize -P tabsize=4 -P mathescape -f latex $^ > $@

code/fmt.tex:
	pygmentize -f latex -S default > $@

fig/%.pdf: fig/%.svg
	inkscape --without-gui -f $^ -D -A $@

data/%.tex: data/%.gp
	BASE=$(basename $@) OUT=$@ TARGET=paper-epslatex gnuplot $<

draft: $(DEPS)
	echo -e '\\newcommand*{\\DRAFT}{}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun $(BTEX) $(MAIN)

watermark: $(DEPS)
	echo -e '\\usepackage[firstpage]{draftwatermark}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun $(BTEX) $(MAIN)

spell:
	@for i in *.tex fig/*.tex; do bin/aspell.sh $$i; done
	@for i in *.tex; do bin/double.pl $$i; done
	@for i in *.tex; do bin/abbrv.pl  $$i; done
	@bin/hyphens.sh *.tex

clean:
	@bin/latexrun --clean
	rm -f abstract.txt

distclean: clean
	rm -f code/*.tex
	rm -f data/*.tex

init:
	rm -f {code,fig,data}/ex-*
	perl -pi -e 's/^\\input{ex}/% \\input{ex}/g' $(MAIN).tex

abstract.txt: abstract.tex $(MAIN).tex
	@bin/mkabstract $(MAIN).tex $< | fmt -w72 > $@

.PHONY: all help FORCE draft clean spell distclean init


==> bin/latexrun <==
#!/usr/bin/env python3

# Copyright (c) 2013, 2014 Austin Clements

# Permission is hereby granted, free of charge, to any person obtaining a copy
# of this software and associated documentation files (the "Software"), to deal
# in the Software without restriction, including without limitation the rights
# to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
# copies of the Software, and to permit persons to whom the Software is
# furnished to do so, subject to the following conditions:

# The above copyright notice and this permission notice shall be included in
# all copies or substantial portions of the Software.

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
# IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
# FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
# AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
# LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
# OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN
# THE SOFTWARE.

import sys
import os
import errno
import argparse
import shlex
import json
import subprocess
import re
import collections
import hashlib
import shutil
import curses
import filecmp
import io
import traceback
import time

try:
    import fcntl
except ImportError:
    # Non-UNIX platform
    fcntl = None

def debug(string, *args):
    if debug.enabled:
        print(string.format(*args), file=sys.stderr)
debug.enabled = False

def debug_exc():
    if debug.enabled:
        traceback.print_exc()

def main():
    # Parse command-line
    arg_parser = argparse.ArgumentParser(
        description='''A 21st century LaTeX wrapper,
        %(prog)s runs latex (and bibtex) the right number of times so you
        don't have to,
        strips the log spew to make errors visible,
        and plays well with standard build tools.''')
    arg_parser.add_argument(
        '-o', metavar='FILE', dest='output', default=None,
        help='Output file name (default: derived from input file)')
    arg_parser.add_argument(
        '--latex-cmd', metavar='CMD', default='pdflatex',
        help='Latex command (default: %(default)s)')
    arg_parser.add_argument(
        '--latex-args', metavar='ARGS', type=arg_parser_shlex,
        help='Additional command-line arguments for latex.'
        ' This will be parsed and split using POSIX shell rules.')
    arg_parser.add_argument(
        '--bibtex-cmd', metavar='CMD', default='bibtex',
        help='Bibtex command (default: %(default)s)')
    arg_parser.add_argument(
        '--bibtex-args', metavar='ARGS', type=arg_parser_shlex,
        help='Additional command-line arguments for bibtex')
    arg_parser.add_argument(
        '--max-iterations', metavar='N', type=int, default=10,
        help='Max number of times to run latex before giving up'
        ' (default: %(default)s)')
    arg_parser.add_argument(
        '-W', metavar='(no-)CLASS',
        action=ArgParserWarnAction, dest='nowarns', default=set(['underfull']),
        help='Enable/disable warning from CLASS, which can be any package name, '
        'LaTeX warning class (e.g., font), bad box type '
        '(underfull, overfull, loose, tight), or "all"')
    arg_parser.add_argument(
        '-O', metavar='DIR', dest='obj_dir', default='latex.out',
        help='Directory for intermediate files and control database '
        '(default: %(default)s)')
    arg_parser.add_argument(
        '--color', choices=('auto', 'always', 'never'), default='auto',
        help='When to colorize messages')
    arg_parser.add_argument(
        '--verbose-cmds', action='store_true', default=False,
        help='Print commands as they are executed')
    arg_parser.add_argument(
        '--debug', action='store_true',
        help='Enable detailed debug output')
    actions = arg_parser.add_argument_group('actions')
    actions.add_argument(
        '--clean-all', action='store_true', help='Delete output files')
    actions.add_argument(
        'file', nargs='?', help='.tex file to compile')
    args = arg_parser.parse_args()
    if not any([args.clean_all, args.file]):
        arg_parser.error('at least one action is required')
    args.latex_args = args.latex_args or []
    args.bibtex_args = args.bibtex_args or []

    verbose_cmd.enabled = args.verbose_cmds
    debug.enabled = args.debug

    # A note about encodings: POSIX encoding is a mess; TeX encoding
    # is a disaster.  Our goal is to make things no worse, so we want
    # byte-accurate round-tripping of TeX messages.  Since TeX
    # messages are *basically* text, we use strings and
    # surrogateescape'ing for both input and output.  I'm not fond of
    # setting surrogateescape globally, but it's far easier than
    # dealing with every place we pass TeX output through.
    # Conveniently, JSON can round-trip surrogateescape'd strings, so
    # our control database doesn't need special handling.
    sys.stdout = io.TextIOWrapper(
        sys.stdout.buffer, encoding=sys.stdout.encoding,
        errors='surrogateescape', line_buffering=sys.stdout.line_buffering)
    sys.stderr = io.TextIOWrapper(
        sys.stderr.buffer, encoding=sys.stderr.encoding,
        errors='surrogateescape', line_buffering=sys.stderr.line_buffering)

    Message.setup_color(args.color)

    # Open control database.
    dbpath = os.path.join(args.obj_dir, '.latexrun.db')
    if not os.path.exists(dbpath) and os.path.exists('.latexrun.db'):
        # The control database used to live in the source directory.
        # Support this for backwards compatibility.
        dbpath = '.latexrun.db'
    try:
        db = DB(dbpath)
    except (ValueError, OSError) as e:
        print('error opening {}: {}'.format(e.filename if hasattr(e, 'filename')
                                            else dbpath, e),
              file=sys.stderr)
        debug_exc()
        sys.exit(1)

    # Clean
    if args.clean_all:
        try:
            db.do_clean(args.obj_dir)
        except OSError as e:
            print(e, file=sys.stderr)
            debug_exc()
            sys.exit(1)

    # Build
    if not args.file:
        return
    task_commit = None
    try:
        task_latex = LaTeX(db, args.file, args.latex_cmd, args.latex_args,
                           args.obj_dir, args.nowarns)
        task_commit = LaTeXCommit(db, task_latex, args.output)
        task_bibtex = BibTeX(db, task_latex, args.bibtex_cmd, args.bibtex_args,
                             args.nowarns, args.obj_dir)
        tasks = [task_latex, task_commit, task_bibtex]
        stable = run_tasks(tasks, args.max_iterations)

        # Print final task output and gather exit status
        status = 0
        for task in tasks:
            status = max(task.report(), status)

        if not stable:
            print('error: files are still changing after {} iterations; giving up'
                  .format(args.max_iterations), file=sys.stderr)
            status = max(status, 1)
    except TaskError as e:
        print(str(e), file=sys.stderr)
        debug_exc()
        status = 1

    # Report final status, if interesting
    fstatus = 'There were errors' if task_commit is None else task_commit.status
    if fstatus:
        output = args.output
        if output is None:
            if task_latex.get_outname() is not None:
                output = os.path.basename(task_latex.get_outname())
            else:
                output = 'output'
        if Message._color:
            terminfo.send('bold', ('setaf', 1))
        print('{}; {} not updated'.format(fstatus, output))
        if Message._color:
            terminfo.send('sgr0')
    sys.exit(status)

def arg_parser_shlex(string):
    """Argument parser for shell token lists."""
    try:
        return shlex.split(string)
    except ValueError as e:
        raise argparse.ArgumentTypeError(str(e)) from None

class ArgParserWarnAction(argparse.Action):
    def __call__(self, parser, namespace, value, option_string=None):
        nowarn = getattr(namespace, self.dest)
        if value == 'all':
            nowarn.clear()
        elif value.startswith('no-'):
            nowarn.add(value[3:])
        else:
            nowarn.discard(value)
        setattr(namespace, self.dest, nowarn)

def verbose_cmd(args, cwd=None, env=None):
    if verbose_cmd.enabled:
        cmd = ' '.join(map(shlex.quote, args))
        if cwd is not None:
            cmd = '(cd {} && {})'.format(shlex.quote(cwd), cmd)
        if env is not None:
            for k, v in env.items():
                if os.environ.get(k) != v:
                    cmd = '{}={} {}'.format(k, shlex.quote(v), cmd)
        print(cmd, file=sys.stderr)
verbose_cmd.enabled = False

def mkdir_p(path):
    try:
        os.makedirs(path)
    except OSError as exc:
        if exc.errno == errno.EEXIST and os.path.isdir(path):
            pass
        else: raise

class DB:
    """A latexrun control database."""

    _VERSION = 'latexrun-db-v2'

    def __init__(self, filename):
        self.__filename = filename

        # Make sure database directory exists
        if os.path.dirname(self.__filename):
            os.makedirs(os.path.dirname(self.__filename), exist_ok=True)

        # Lock the database if possible. We don't release this lock
        # until the process exits.
        lockpath = self.__filename + '.lock'
        if fcntl is not None:
            lockfd = os.open(lockpath, os.O_CREAT|os.O_WRONLY|os.O_CLOEXEC, 0o666)
            # Note that this is actually an fcntl lock, not a lockf
            # lock. Don't be fooled.
            fcntl.lockf(lockfd, fcntl.LOCK_EX, 1)

        try:
            fp = open(filename, 'r')
        except FileNotFoundError:
            debug('creating new database')
            self.__val = {'version': DB._VERSION}
        else:
            debug('loading database')
            self.__val = json.load(fp)
            if 'version' not in self.__val:
                raise ValueError('file exists, but does not appear to be a latexrun database'.format(filename))
            if self.__val['version'] != DB._VERSION:
                raise ValueError('unknown database version {!r}'
                                 .format(self.__val['version']))

    def commit(self):
        debug('committing database')
        # Atomically commit database
        tmp_filename = self.__filename + '.tmp'
        with open(tmp_filename, 'w') as fp:
            json.dump(self.__val, fp, indent=2, separators=(',', ': '))
            fp.flush()
            os.fsync(fp.fileno())
        os.rename(tmp_filename, self.__filename)

    def get_summary(self, task_id):
        """Return the recorded summary for the given task or None."""
        return self.__val.get('tasks', {}).get(task_id)

    def set_summary(self, task_id, summary):
        """Set the summary for the given task."""
        self.__val.setdefault('tasks', {})[task_id] = summary

    def add_clean(self, filename):
        """Add an output file to be cleaned.

        Unlike the output files recorded in the task summaries,
        cleanable files strictly accumulate until a clean is
        performed.
        """
        self.__val.setdefault('clean', {})[filename] = hash_cache.get(filename)

    def do_clean(self, obj_dir=None):
        """Remove output files and delete database.

        If obj_dir is not None and it is empty after all files are
        removed, it will also be removed.
        """

        for f, want_hash in self.__val.get('clean', {}).items():
            have_hash = hash_cache.get(f)
            if have_hash is not None:
                if want_hash == have_hash:
                    debug('unlinking {}', f)
                    hash_cache.invalidate(f)
                    os.unlink(f)
                else:
                    print('warning: {} has changed; not removing'.format(f),
                          file=sys.stderr)
        self.__val = {'version': DB._VERSION}
        try:
            os.unlink(self.__filename)
        except FileNotFoundError:
            pass
        if obj_dir is not None:
            try:
                os.rmdir(obj_dir)
            except OSError:
                pass

class HashCache:
    """Cache of file hashes.

    As latexrun reaches fixed-point, it hashes the same files over and
    over, many of which never change.  Since hashing is somewhat
    expensive, we keep a simple cache of these hashes.
    """

    def __init__(self):
        self.__cache = {}

    def get(self, filename):
        """Return the hash of filename, or * if it was clobbered."""
        try:
            with open(filename, 'rb') as fp:
                st = os.fstat(fp.fileno())
                key = (st.st_dev, st.st_ino)
                if key in self.__cache:
                    return self.__cache[key]

                debug('hashing {}', filename)
                h = hashlib.sha256()
                while True:
                    block = fp.read(256*1024)
                    if not len(block):
                        break
                    h.update(block)
                self.__cache[key] = h.hexdigest()
                return self.__cache[key]
        except (FileNotFoundError, IsADirectoryError):
            return None

    def clobber(self, filename):
        """If filename's hash is not known, record an invalid hash.

        This can be used when filename was overwritten before we were
        necessarily able to obtain its hash.  filename must exist.
        """
        st = os.stat(filename)
        key = (st.st_dev, st.st_ino)
        if key not in self.__cache:
            self.__cache[key] = '*'

    def invalidate(self, filename):
        try:
            st = os.stat(filename)
        except OSError as e:
            # Pessimistically wipe the whole cache
            debug('wiping hash cache ({})', e)
            self.__cache.clear()
        else:
            key = (st.st_dev, st.st_ino)
            if key in self.__cache:
                del self.__cache[key]
hash_cache = HashCache()

class _Terminfo:
    def __init__(self):
        self.__tty = os.isatty(sys.stdout.fileno())
        if self.__tty:
            curses.setupterm()
        self.__ti = {}

    def __ensure(self, cap):
        if cap not in self.__ti:
            if not self.__tty:
                string = None
            else:
                string = curses.tigetstr(cap)
                if string is None or b'$<' in string:
                    # Don't have this capability or it has a pause
                    string = None
            self.__ti[cap] = string
        return self.__ti[cap]

    def has(self, *caps):
        return all(self.__ensure(cap) is not None for cap in caps)

    def send(self, *caps):
        # Flush TextIOWrapper to the binary IO buffer
        sys.stdout.flush()
        for cap in caps:
            # We should use curses.putp here, but it's broken in
            # Python3 because it writes directly to C's buffered
            # stdout and there's no way to flush that.
            if isinstance(cap, tuple):
                s = curses.tparm(self.__ensure(cap[0]), *cap[1:])
            else:
                s = self.__ensure(cap)
            sys.stdout.buffer.write(s)
terminfo = _Terminfo()

class Progress:
    _enabled = None

    def __init__(self, prefix):
        self.__prefix = prefix
        if Progress._enabled is None:
            Progress._enabled = (not debug.enabled) and \
                                terminfo.has('cr', 'el', 'rmam', 'smam')

    def __enter__(self):
        self.last = ''
        self.update('')
        return self

    def __exit__(self, typ, value, traceback):
        if Progress._enabled:
            # Beginning of line and clear
            terminfo.send('cr', 'el')
            sys.stdout.flush()

    def update(self, msg):
        if not Progress._enabled:
            return
        out = '[' + self.__prefix + ']'
        if msg:
            out += ' ' + msg
        if out != self.last:
            # Beginning of line, clear line, disable wrap
            terminfo.send('cr', 'el', 'rmam')
            sys.stdout.write(out)
            # Enable wrap
            terminfo.send('smam')
            self.last = out
            sys.stdout.flush()

class Message(collections.namedtuple(
        'Message', 'typ filename lineno msg')):
    def emit(self):
        if self.filename:
            if self.filename.startswith('./'):
                finfo = self.filename[2:]
            else:
                finfo = self.filename
        else:
            finfo = '<no file>'
        if self.lineno is not None:
            finfo += ':' + str(self.lineno)
        finfo += ': '
        if self._color:
            terminfo.send('bold')
        sys.stdout.write(finfo)

        if self.typ != 'info':
            if self._color:
                terminfo.send(('setaf', 5 if self.typ == 'warning' else 1))
            sys.stdout.write(self.typ + ': ')
        if self._color:
            terminfo.send('sgr0')
        sys.stdout.write(self.msg + '\n')

    @classmethod
    def setup_color(cls, state):
        if state == 'never':
            cls._color = False
        elif state == 'always':
            cls._color = True
        elif state == 'auto':
            cls._color = terminfo.has('setaf', 'bold', 'sgr0')
        else:
            raise ValueError('Illegal color state {:r}'.format(state))


##################################################################
# Task framework
#

terminate_task_loop = False
start_time = time.time()

def run_tasks(tasks, max_iterations):
    """Execute tasks in round-robin order until all are stable.

    This will also exit if terminate_task_loop is true.  Tasks may use
    this to terminate after a fatal error (even if that fatal error
    doesn't necessarily indicate stability; as long as re-running the
    task will never eliminate the fatal error).

    Return True if fixed-point is reached or terminate_task_loop is
    set within max_iterations iterations.
    """

    global terminate_task_loop
    terminate_task_loop = False

    nstable = 0
    for iteration in range(max_iterations):
        for task in tasks:
            if task.stable():
                nstable += 1
                if nstable == len(tasks):
                    debug('fixed-point reached')
                    return True
            else:
                task.run()
                nstable = 0
                if terminate_task_loop:
                    debug('terminate_task_loop set')
                    return True
    debug('fixed-point not reached')
    return False

class TaskError(Exception):
    pass

class Task:
    """A deterministic computation whose inputs and outputs can be captured."""

    def __init__(self, db, task_id):
        self.__db = db
        self.__task_id = task_id

    def __debug(self, string, *args):
        if debug.enabled:
            debug('task {}: {}', self.__task_id, string.format(*args))

    def stable(self):
        """Return True if running this task will not affect system state.

        Functionally, let f be the task, and s be the system state.
        Then s' = f(s).  If it must be that s' == s (that is, f has
        reached a fixed point), then this function must return True.
        """
        last_summary = self.__db.get_summary(self.__task_id)
        if last_summary is None:
            # Task has never run, so running it will modify system
            # state
            changed = 'never run'
        else:
            # If any of the inputs have changed since the last run of
            # this task, the result may change, so re-run the task.
            # Also, it's possible something else changed an output
            # file, in which case we also want to re-run the task, so
            # check the outputs, too.
            changed = self.__summary_changed(last_summary)

        if changed:
            self.__debug('unstable (changed: {})', changed)
            return False
        else:
            self.__debug('stable')
            return True

    def __summary_changed(self, summary):
        """Test if any inputs changed from summary.

        Returns a string describing the changed input, or None.
        """
        for dep in summary['deps']:
            fn, args, val = dep
            method = getattr(self, '_input_' + fn, None)
            if method is None:
                return 'unknown dependency method {}'.format(fn)
            if method == self._input_unstable or method(*args) != val:
                return '{}{}'.format(fn, tuple(args))
        return None

    def _input(self, name, *args):
        """Register an input for this run.

        This calls self._input_<name>(*args) to get the value of this
        input.  This function should run quickly and return some
        projection of system state that affects the result of this
        computation.

        Both args and the return value must be JSON serializable.
        """
        method = getattr(self, '_input_' + name)
        val = method(*args)
        if [name, args, val] not in self.__deps:
            self.__deps.append([name, args, val])
        return val

    def run(self):
        # Before we run the task, pre-hash any files that were output
        # files in the last run.  These may be input by this run and
        # then clobbered, at which point it will be too late to get an
        # input hash.  Ideally we would only hash files that were
        # *both* input and output files, but latex doesn't tell us
        # about input files that didn't exist, so if we start from a
        # clean slate, we often require an extra run because we don't
        # know a file is input/output until after the second run.
        last_summary = self.__db.get_summary(self.__task_id)
        if last_summary is not None:
            for io_filename in last_summary['output_files']:
                self.__debug('pre-hashing {}', io_filename)
                hash_cache.get(io_filename)

        # Run the task
        self.__debug('running')
        self.__deps = []
        result = self._execute()

        # Clear cached output file hashes
        for filename in result.output_filenames:
            hash_cache.invalidate(filename)

        # If the output files change, then the computation needs to be
        # re-run, so record them as inputs
        for filename in result.output_filenames:
            self._input('file', filename)

        # Update task summary in database
        self.__db.set_summary(self.__task_id,
                              self.__make_summary(self.__deps, result))
        del self.__deps

        # Add output files to be cleaned
        for f in result.output_filenames:
            self.__db.add_clean(f)

        try:
            self.__db.commit()
        except OSError as e:
            raise TaskError('error committing control database {}: {}'.format(
                getattr(e, 'filename', '<unknown path>'), e)) from e

    def __make_summary(self, deps, run_result):
        """Construct a new task summary."""
        return {
            'deps': deps,
            'output_files': {f: hash_cache.get(f)
                             for f in run_result.output_filenames},
            'extra': run_result.extra,
        }

    def _execute(self):
        """Abstract: Execute this task.

        Subclasses should implement this method to execute this task.
        This method must return a RunResult giving the inputs that
        were used by the task and the outputs it produced.
        """
        raise NotImplementedError('Task._execute is abstract')

    def _get_result_extra(self):
        """Return the 'extra' result from the previous run, or None."""
        summary = self.__db.get_summary(self.__task_id)
        if summary is None:
            return None
        return summary['extra']

    def report(self):
        """Report the task's results to stdout and return exit status.

        This may be called when the task has never executed.
        Subclasses should override this.  The default implementation
        reports nothing and returns 0.
        """
        return 0

    # Standard input functions

    def _input_env(self, var):
        return os.environ.get(var)

    def _input_file(self, path):
        return hash_cache.get(path)

    def _input_unstable(self):
        """Mark this run as unstable, regardless of other inputs."""
        return None

    def _input_unknown_input(self):
        """An unknown input that may change after latexrun exits.

        This conservatively marks some unknown input that definitely
        won't change while latexrun is running, but may change before
        the user next runs latexrun.  This allows the task to
        stabilize during this invocation, but will cause the task to
        re-run on the next invocation.
        """
        return start_time

class RunResult(collections.namedtuple(
        'RunResult', 'output_filenames extra')):
    """The result of a single task execution.

    This captures all files written by the task, and task-specific
    results that need to be persisted between runs (for example, to
    enable reporting of a task's results).
    """
    pass

##################################################################
# LaTeX task
#

def normalize_input_path(path):
    # Resolve the directory of the input path, but leave the file
    # component alone because it affects TeX's behavior.
    head, tail = os.path.split(path)
    npath = os.path.join(os.path.realpath(head), tail)
    return os.path.relpath(path)

class LaTeX(Task):
    def __init__(self, db, tex_filename, cmd, cmd_args, obj_dir, nowarns):
        super().__init__(db, 'latex::' + normalize_input_path(tex_filename))
        self.__tex_filename = tex_filename
        self.__cmd = cmd
        self.__cmd_args = cmd_args
        self.__obj_dir = obj_dir
        self.__nowarns = nowarns

        self.__pass = 0

    def _input_args(self):
        # If filename starts with a character the tex command-line
        # treats specially, then tweak it so it doesn't.
        filename = self.__tex_filename
        if filename.startswith(('-', '&', '\\')):
            filename = './' + filename
        # XXX Put these at the beginning in case the provided
        # arguments are malformed.  Might want to do a best-effort
        # check for incompatible user-provided arguments (note:
        # arguments can be given with one or two dashes and those with
        # values can use an equals or a space).
        return [self.__cmd] + self.__cmd_args + \
            ['-interaction', 'nonstopmode', '-recorder',
             '-output-directory', self.__obj_dir, filename]

    def _execute(self):
        # Run latex
        self.__pass += 1
        args = self._input('args')
        debug('running {}', args)
        try:
            os.makedirs(self.__obj_dir, exist_ok=True)
        except OSError as e:
            raise TaskError('failed to create %s: ' % self.__obj_dir + str(e)) \
                from e
        try:
            verbose_cmd(args)
            p = subprocess.Popen(args,
                                 stdin=subprocess.DEVNULL,
                                 stdout=subprocess.PIPE,
                                 stderr=subprocess.STDOUT)
            stdout, has_errors, missing_includes = self.__feed_terminal(p.stdout)
            status = p.wait()
        except OSError as e:
            raise TaskError('failed to execute latex task: ' + str(e)) from e

        # Register environment variable inputs
        for env_var in ['TEXMFOUTPUT', 'TEXINPUTS', 'TEXFORMATS', 'TEXPOOL',
                        'TFMFONTS', 'PATH']:
            self._input('env', env_var)

        jobname, outname = self.__parse_jobname(stdout)
        inputs, outputs = self.__parse_recorder(jobname)

        # LaTeX overwrites its own inputs.  Mark its output files as
        # clobbered before we hash its input files.
        for path in outputs:
            # In some abort cases (e.g., >=100 errors), LaTeX claims
            # output files that don't actually exist.
            if os.path.exists(path):
                hash_cache.clobber(path)
        # Depend on input files.  Task.run pre-hashed outputs from the
        # previous run, so if this isn't the first run and as long as
        # the set of outputs didn't change, we'll be able to get the
        # input hashes, even if they were clobbered.
        for path in inputs:
            self._input('file', path)

        if missing_includes:
            # Missing \includes are tricky.  Ideally we'd depend on
            # the absence of some file, but in fact we'd have to
            # depend on the failure of a whole kpathsea lookup.
            # Rather than try to be clever, just mark this as an
            # unknown input so we'll run at least once on the next
            # invocation.
            self._input('unknown_input')

        if not self.__create_outdirs(stdout) and has_errors:
            # LaTeX reported unrecoverable errors (other than output
            # directory errors, which we just fixed).  We could
            # continue to stabilize the document, which may change
            # some of the other problems reported (but not the
            # unrecoverable errors), or we can just abort now and get
            # back to the user quickly with the major errors.  We opt
            # for the latter.
            global terminate_task_loop
            terminate_task_loop = True
            # This error could depend on something we failed to track.
            # It would be really confusing if we continued to report
            # the error after the user fixed it, so be conservative
            # and force a re-run next time.
            self._input('unknown_input')

        return RunResult(outputs,
                         {'jobname': jobname, 'outname': outname,
                          'status': status})

    def __feed_terminal(self, stdout):
        prefix = 'latex'
        if self.__pass > 1:
            prefix += ' ({})'.format(self.__pass)
        with Progress(prefix) as progress:
            buf = []
            filt = LaTeXFilter()
            while True:
                # Use os.read to read only what's available on the pipe,
                # without waiting to fill a buffer
                data = os.read(stdout.fileno(), 4096)
                if not data:
                    break
                # See "A note about encoding" above
                data = data.decode('ascii', errors='surrogateescape')
                buf.append(data)
                filt.feed(data)
                file_stack = filt.get_file_stack()
                if file_stack:
                    tos = file_stack[-1]
                    if tos.startswith('./'):
                        tos = tos[2:]
                    progress.update('>' * len(file_stack) + ' ' + tos)
                else:
                    progress.update('')

            # Were there unrecoverable errors?
            has_errors = any(msg.typ == 'error' for msg in filt.get_messages())

            return ''.join(buf), has_errors, filt.has_missing_includes()

    def __parse_jobname(self, stdout):
        """Extract the job name and output name from latex's output.

        We get these from latex because they depend on complicated
        file name parsing rules, are affected by arguments like
        -output-directory, and may be just "texput" if things fail
        really early.  The output name may be None if there were no
        pages of output.
        """
        jobname = outname = None
        for m in re.finditer(r'^Transcript written on "?(.*)\.log"?\.$', stdout,
                             re.MULTILINE | re.DOTALL):
            jobname = m.group(1).replace('\n', '')
        if jobname is None:
            print(stdout, file=sys.stderr)
            raise TaskError('failed to extract job name from latex log')
        for m in re.finditer(r'^Output written on "?(.*\.[^ ."]+)"? \([0-9]+ page',
                             stdout, re.MULTILINE | re.DOTALL):
            outname = m.group(1).replace('\n', '')
        if outname is None and not \
           re.search(r'^No pages of output\.$|^! Emergency stop\.$'
                     r'|^!  ==> Fatal error occurred, no output PDF file produced!$',
                     stdout, re.MULTILINE):
            print(stdout, file=sys.stderr)
            raise TaskError('failed to extract output name from latex log')

        # LuaTeX (0.76.0) doesn't include the output directory in the
        # logged transcript or output file name.
        if os.path.basename(jobname) == jobname and \
           os.path.exists(os.path.join(self.__obj_dir, jobname + '.log')):
            jobname = os.path.join(self.__obj_dir, jobname)
            if outname is not None:
                outname = os.path.join(self.__obj_dir, outname)

        return jobname, outname

    def __parse_recorder(self, jobname):
        """Parse file recorder output."""
        # XXX If latex fails because a file isn't found, that doesn't
        # go into the .fls file, but creating that file will affect
        # the computation, so it should be included as an input.
        # Though it's generally true that files can be added earlier
        # in search paths and will affect the output without us knowing.
        #
        # XXX This is a serious problem for bibtex, since the first
        # run won't depend on the .bbl file!  But maybe the .aux file
        # will always cause a re-run, at which point the .bbl will
        # exist?
        filename = jobname + '.fls'
        try:
            recorder = open(filename)
        except OSError as e:
            raise TaskError('failed to open file recorder output: ' + str(e)) \
                from e
        pwd, inputs, outputs = '', set(), set()
        for linenum, line in enumerate(recorder):
            parts = line.rstrip('\n').split(' ', 1)
            if parts[0] == 'PWD':
                pwd = parts[1]
            elif parts[0] in ('INPUT', 'OUTPUT'):
                if parts[1].startswith('/'):
                    path = parts[1]
                else:
                    # Try to make "nice" paths, especially for clean
                    path = os.path.relpath(os.path.join(pwd, parts[1]))
                if parts[0] == 'INPUT':
                    inputs.add(path)
                else:
                    outputs.add(path)
            else:
                raise TaskError('syntax error on line {} of {}'
                                .format(linenum, filename))
        # Ironically, latex omits the .fls file itself
        outputs.add(filename)
        return inputs, outputs

    def __create_outdirs(self, stdout):
        # In some cases, such as \include'ing a file from a
        # subdirectory, TeX will attempt to create files in
        # subdirectories of the output directory that don't exist.
        # Detect this, create the output directory, and re-run.
        m = re.search('^! I can\'t write on file `(.*)\'\\.$', stdout, re.M)
        if m and m.group(1).find('/') > 0 and '../' not in m.group(1):
            debug('considering creating output sub-directory for {}'.
                  format(m.group(1)))
            subdir = os.path.dirname(m.group(1))
            newdir = os.path.join(self.__obj_dir, subdir)
            if os.path.isdir(subdir) and not os.path.isdir(newdir):
                debug('creating output subdirectory {}'.format(newdir))
                try:
                    mkdir_p(newdir)
                except OSError as e:
                    raise TaskError('failed to create output subdirectory: ' +
                                    str(e)) from e
                self._input('unstable')
                return True

    def report(self):
        extra = self._get_result_extra()
        if extra is None:
            return 0

        # Parse the log
        logfile = open(extra['jobname'] + '.log', 'rt', errors='surrogateescape')
        for msg in self.__clean_messages(
                LaTeXFilter(self.__nowarns).feed(
                    logfile.read(), True).get_messages()):
            msg.emit()

        # Return LaTeX's exit status
        return extra['status']

    def __clean_messages(self, msgs):
        """Make some standard log messages more user-friendly."""
        have_undefined_reference = False
        for msg in msgs:
            if msg.msg == '==> Fatal error occurred, no output PDF file produced!':
                msg = msg._replace(typ='info',
                                   msg='Fatal error (no output file produced)')
            if msg.msg.startswith('[LaTeX] '):
                # Strip unnecessary package name
                msg = msg._replace(msg=msg.msg.split(' ', 1)[1])
            if re.match(r'Reference .* undefined', msg.msg):
                have_undefined_reference = True
            if have_undefined_reference and \
               re.match(r'There were undefined references', msg.msg):
                # LaTeX prints this at the end so the user knows it's
                # worthwhile looking back at the log.  Since latexrun
                # makes the earlier messages obvious, this is
                # redundant.
                continue
            yield msg

    def get_tex_filename(self):
        return self.__tex_filename

    def get_jobname(self):
        extra = self._get_result_extra()
        if extra is None:
            return None
        return extra['jobname']

    def get_outname(self):
        extra = self._get_result_extra()
        if extra is None:
            return None
        return extra['outname']

    def get_status(self):
        extra = self._get_result_extra()
        if extra is None:
            return None
        return extra['status']

class LaTeXCommit(Task):
    def __init__(self, db, latex_task, output_path):
        super().__init__(db, 'latex_commit::' +
                         normalize_input_path(latex_task.get_tex_filename()))
        self.__latex_task = latex_task
        self.__output_path = output_path
        self.status = 'There were errors'

    def _input_latex(self):
        return self.__latex_task.get_status(), self.__latex_task.get_outname()

    def _execute(self):
        self.status = 'There were errors'

        # If latex succeeded with output, atomically commit the output
        status, outname = self._input('latex')
        if status != 0 or outname is None:
            debug('not committing (status {}, outname {})', status, outname)
            if outname is None:
                self.status = 'No pages of output'
            return RunResult([], None)

        commit = self.__output_path or os.path.basename(outname)
        if os.path.abspath(commit) == os.path.abspath(outname):
            debug('skipping commit (outname is commit name)')
            self.status = None
            return RunResult([], None)

        try:
            if os.path.exists(commit) and filecmp.cmp(outname, commit):
                debug('skipping commit ({} and {} are identical)',
                      outname, commit)
                # To avoid confusion, touch the output file
                open(outname, 'r+b').close()
            else:
                debug('commiting {} to {}', outname, commit)
                shutil.copy(outname, outname + '~')
                os.rename(outname + '~', commit)
        except OSError as e:
            raise TaskError('error committing latex output: {}'.format(e)) from e
        self._input('file', outname)
        self.status = None
        return RunResult([commit], None)

class LaTeXFilter:
    TRACE = False               # Set to enable detailed parse tracing

    def __init__(self, nowarns=[]):
        self.__data = ''
        self.__restart_pos = 0
        self.__restart_file_stack = []
        self.__restart_messages_len = 0
        self.__messages = []
        self.__first_file = None
        self.__fatal_error = False
        self.__missing_includes = False
        self.__pageno = 1
        self.__restart_pageno = 1

        self.__suppress = {cls: 0 for cls in nowarns}

    def feed(self, data, eof=False):
        """Feed LaTeX log data to the parser.

        The log data can be from LaTeX's standard output, or from the
        log file.  If there will be no more data, set eof to True.
        """

        self.__data += data
        self.__data_complete = eof

        # Reset to last known-good restart point
        self.__pos = self.__restart_pos
        self.__file_stack = self.__restart_file_stack.copy()
        self.__messages = self.__messages[:self.__restart_messages_len]
        self.__lstart = self.__lend = -1
        self.__pageno = self.__restart_pageno

        # Parse forward
        while self.__pos < len(self.__data):
            self.__noise()

        # Handle suppressed warnings
        if eof:
            msgs = ['%d %s warning%s' % (count, cls, "s" if count > 1 else "")
                    for cls, count in self.__suppress.items() if count]
            if msgs:
                self.__message('info', None,
                               '%s not shown (use -Wall to show them)' %
                               ', '.join(msgs), filename=self.__first_file)

        if eof and len(self.__file_stack) and not self.__fatal_error:
            # Fatal errors generally cause TeX to "succumb" without
            # closing the file stack, so don't complain in that case.
            self.__message('warning', None,
                           "unbalanced `(' in log; file names may be wrong")
        return self

    def get_messages(self):
        """Return a list of warning and error Messages."""
        return self.__messages

    def get_file_stack(self):
        """Return the file stack for the data that has been parsed.

        This results a list from outermost file to innermost file.
        The list may be empty.
        """

        return self.__file_stack

    def has_missing_includes(self):
        """Return True if the log reported missing \\include files."""
        return self.__missing_includes

    def __save_restart_point(self):
        """Save the current state as a known-good restart point.

        On the next call to feed, the parser will reset to this point.
        """
        self.__restart_pos = self.__pos
        self.__restart_file_stack = self.__file_stack.copy()
        self.__restart_messages_len = len(self.__messages)
        self.__restart_pageno = self.__pageno

    def __message(self, typ, lineno, msg, cls=None, filename=None):
        if cls is not None and cls in self.__suppress:
            self.__suppress[cls] += 1
            return
        filename = filename or (self.__file_stack[-1] if self.__file_stack
                                else self.__first_file)
        self.__messages.append(Message(typ, filename, lineno, msg))

    def __ensure_line(self):
        """Update lstart and lend."""
        if self.__lstart <= self.__pos < self.__lend:
            return
        self.__lstart = self.__data.rfind('\n', 0, self.__pos) + 1
        self.__lend = self.__data.find('\n', self.__pos) + 1
        if self.__lend == 0:
            self.__lend = len(self.__data)

    @property
    def __col(self):
        """The 0-based column number of __pos."""
        self.__ensure_line()
        return self.__pos - self.__lstart

    @property
    def __avail(self):
        return self.__pos < len(self.__data)

    def __lookingat(self, needle):
        return self.__data.startswith(needle, self.__pos)

    def __lookingatre(self, regexp, flags=0):
        return re.compile(regexp, flags=flags).match(self.__data, self.__pos)

    def __skip_line(self):
        self.__ensure_line()
        self.__pos = self.__lend

    def __consume_line(self, unwrap=False):
        self.__ensure_line()
        data = self.__data[self.__pos:self.__lend]
        self.__pos = self.__lend
        if unwrap:
            # TeX helpfully wraps all terminal output at 79 columns
            # (max_print_line).  If requested, unwrap it.  There's
            # simply no way to do this perfectly, since there could be
            # a line that happens to be 79 columns.
            #
            # We check for >=80 because a bug in LuaTeX causes it to
            # wrap at 80 columns instead of 79 (LuaTeX #900).
            while self.__lend - self.__lstart >= 80:
                if self.TRACE: print('<{}> wrapping'.format(self.__pos))
                self.__ensure_line()
                data = data[:-1] + self.__data[self.__pos:self.__lend]
                self.__pos = self.__lend
        return data

    # Parser productions

    def __noise(self):
        # Most of TeX's output is line noise that combines error
        # messages, warnings, file names, user errors and warnings,
        # and echos of token lists and other input.  This attempts to
        # tease these apart, paying particular attention to all of the
        # places where TeX echos input so that parens in the input do
        # not confuse the file name scanner.  There are three
        # functions in TeX that echo input: show_token_list (used by
        # runaway and show_context, which is used by print_err),
        # short_display (used by overfull/etc h/vbox), and show_print
        # (used in issue_message and the same places as
        # show_token_list).
        lookingat, lookingatre = self.__lookingat, self.__lookingatre
        if self.__col == 0:
            # The following messages are always preceded by a newline
            if lookingat('! '):
                return self.__errmessage()
            if lookingat('!pdfTeX error: '):
                return self.__pdftex_fail()
            if lookingat('Runaway '):
                return self.__runaway()
            if lookingatre(r'(Overfull|Underfull|Loose|Tight) \\[hv]box \('):
                return self.__bad_box()
            if lookingatre('(Package |Class |LaTeX |pdfTeX )?(\w+ )?warning: ', re.I):
                return self.__generic_warning()
            if lookingatre('No file .*\\.tex\\.$', re.M):
                # This happens with \includes of missing files.  For
                # whatever reason, LaTeX doesn't consider this even
                # worth a warning, but I do!
                self.__message('warning', None,
                               self.__simplify_message(
                                   self.__consume_line(unwrap=True).strip()))
                self.__missing_includes = True
                return
            # Other things that are common and irrelevant
            if lookingatre(r'(Package|Class|LaTeX) (\w+ )?info: ', re.I):
                return self.__generic_info()
            if lookingatre(r'(Document Class|File|Package): '):
                # Output from "\ProvidesX"
                return self.__consume_line(unwrap=True)
            if lookingatre(r'\\\w+=\\[a-z]+\d+\n'):
                # Output from "\new{count,dimen,skip,...}"
                return self.__consume_line(unwrap=True)

        # print(self.__data[self.__lstart:self.__lend].rstrip())
        # self.__pos = self.__lend
        # return

        # Now that we've substantially reduced the spew and hopefully
        # eliminated all input echoing, we're left with the file name
        # stack, page outs, and random other messages from both TeX
        # and various packages.  We'll assume at this point that all
        # parentheses belong to the file name stack or, if they're in
        # random other messages, they're at least balanced and nothing
        # interesting happens between them.  For page outs, ship_out
        # prints a space if not at the beginning of a line, then a
        # "[", then the page number being shipped out (this is
        # usually, but not always, followed by "]").
        m = re.compile(r'[(){}\n]|(?<=[\n ])\[\d+', re.M).\
            search(self.__data, self.__pos)
        if m is None:
            self.__pos = len(self.__data)
            return
        self.__pos = m.start() + 1
        ch = self.__data[m.start()]
        if ch == '\n':
            # Save this as a known-good restart point for incremental
            # parsing, since we definitely didn't match any of the
            # known message types above.
            self.__save_restart_point()
        elif ch == '[':
            # This is printed at the end of a page, so we're beginning
            # page n+1.
            self.__pageno = int(self.__lookingatre(r'\d+').group(0)) + 1
        elif ((self.__data.startswith('`', m.start() - 1) or
               self.__data.startswith('`\\', m.start() - 2)) and
               self.__data.startswith('\'', m.start() + 1)):
            # (, ), {, and } sometimes appear in TeX's error
            # descriptions, but they're always in `'s (and sometimes
            # backslashed)
            return
        elif ch == '(':
            # XXX Check that the stack doesn't drop to empty and then re-grow
            first = self.__first_file is None and self.__col == 1
            filename = self.__filename()
            self.__file_stack.append(filename)
            if first:
                self.__first_file = filename
            if self.TRACE:
                print('<{}>{}enter {}'.format(
                    m.start(), ' '*len(self.__file_stack), filename))
        elif ch == ')':
            if len(self.__file_stack):
                if self.TRACE:
                    print('<{}>{}exit {}'.format(
                        m.start(), ' '*len(self.__file_stack),
                        self.__file_stack[-1]))
                self.__file_stack.pop()
            else:
                self.__message('warning', None,
                               "extra `)' in log; file names may be wrong ")
        elif ch == '{':
            # TeX uses this for various things we want to ignore, like
            # file names and print_mark.  Consume up to the '}'
            epos = self.__data.find('}', self.__pos)
            if epos != -1:
                self.__pos = epos + 1
            else:
                self.__message('warning', None,
                               "unbalanced `{' in log; file names may be wrong")
        elif ch == '}':
            self.__message('warning', None,
                           "extra `}' in log; file names may be wrong")

    def __filename(self):
        initcol = self.__col
        first = True
        name = ''
        # File names may wrap, but if they do, TeX will always print a
        # newline before the open paren
        while first or (initcol == 1 and self.__lookingat('\n')
                        and self.__col >= 79):
            if not first:
                self.__pos += 1
            m = self.__lookingatre(r'[^(){} \n]*')
            name += m.group()
            self.__pos = m.end()
            first = False
        return name

    def __simplify_message(self, msg):
        msg = re.sub(r'^(?:Package |Class |LaTeX |pdfTeX )?([^ ]+) (?:Error|Warning): ',
                     r'[\1] ', msg, flags=re.I)
        msg = re.sub(r'\.$', '', msg)
        msg = re.sub(r'has occurred (while \\output is active)', r'\1', msg)
        return msg

    def __errmessage(self):
        # Procedure print_err (including \errmessage, itself used by
        # LaTeX's \GenericError and all of its callers), as well as
        # fatal_error.  Prints "\n!  " followed by error text
        # ("Emergency stop" in the case of fatal_error).  print_err is
        # always followed by a call to error, which prints a period,
        # and a newline...
        msg = self.__consume_line(unwrap=True)[1:].strip()
        is_fatal_error = (msg == 'Emergency stop.')
        msg = self.__simplify_message(msg)
        # ... and then calls show_context, which prints the input
        # stack as pairs of lines giving the context.  These context
        # lines are truncated so they never wrap.  Each pair of lines
        # will start with either "<something> " if the context is a
        # token list, "<*> " for terminal input (or command line),
        # "<read ...>" for stream reads, something like "\macroname
        # #1->" for macros (though everything after \macroname is
        # subject to being elided as "..."), or "l.[0-9]+ " if it's a
        # file.  This is followed by the errant input with a line
        # break where the error occurred.
        lineno = None
        found_context = False
        stack = []
        while self.__avail:
            m1 = self.__lookingatre(r'<([a-z ]+|\*|read [^ >]*)> |\\.*(->|...)')
            m2 = self.__lookingatre('l\.[0-9]+ ')
            if m1:
                found_context = True
                pre = self.__consume_line().rstrip('\n')
                stack.append(pre)
            elif m2:
                found_context = True
                pre = self.__consume_line().rstrip('\n')
                info, rest = pre.split(' ', 1)
                lineno = int(info[2:])
                stack.append(rest)
            elif found_context:
                # Done with context
                break
            if found_context:
                # Consume the second context line
                post = self.__consume_line().rstrip('\n')
                # Clean up goofy trailing ^^M TeX sometimes includes
                post = re.sub(r'\^\^M$', '', post)
                if post[:len(pre)].isspace() and not post.isspace():
                    stack.append(len(stack[-1]))
                    stack[-2] += post[len(pre):]
            else:
                # If we haven't found the context, skip the line.
                self.__skip_line()
        stack_msg = ''
        for i, trace in enumerate(stack):
            stack_msg += ('\n         ' + (' ' * trace) + '^'
                          if isinstance(trace, int) else
                          '\n      at ' + trace.rstrip() if i == 0 else
                          '\n    from ' + trace.rstrip())

        if is_fatal_error:
            # fatal_error always prints one additional line of message
            info = self.__consume_line().strip()
            if info.startswith('*** '):
                info = info[4:]
            msg += ': '  + info.lstrip('(').rstrip(')')

        self.__message('error', lineno, msg + stack_msg)
        self.__fatal_error = True

    def __pdftex_fail(self):
        # Procedure pdftex_fail.  Prints "\n!pdfTeX error: ", the
        # message, and a newline.  Unlike print_err, there's never
        # context.
        msg = self.__consume_line(unwrap=True)[1:].strip()
        msg = self.__simplify_message(msg)
        self.__message('error', None, msg)

    def __runaway(self):
        # Procedure runaway.  Prints "\nRunaway ...\n" possibly
        # followed by token list (user text).  Always followed by a
        # call to print_err, so skip lines until we see the print_err.
        self.__skip_line()      # Skip "Runaway ...\n"
        if not self.__lookingat('! ') and self.__avail:
            # Skip token list, which is limited to one line
            self.__skip_line()

    def __bad_box(self):
        # Function hpack and vpack.  hpack prints a warning, a
        # newline, then a short_display of the offending text.
        # Unfortunately, there's nothing indicating the end of the
        # offending text, but it should be on one (possible wrapped)
        # line.  vpack prints a warning and then, *unless output is
        # active*, a newline.  The missing newline is probably a bug,
        # but it sure makes our lives harder.
        origpos = self.__pos
        msg = self.__consume_line()
        m = re.search(r' in (?:paragraph|alignment) at lines ([0-9]+)--([0-9]+)', msg) or \
            re.search(r' detected at line ([0-9]+)', msg)
        if m:
            # Sometimes TeX prints crazy line ranges like "at lines
            # 8500--250".  The lower number seems roughly sane, so use
            # that.  I'm not sure what causes this, but it may be
            # related to shipout routines messing up line registers.
            lineno = min(int(m.group(1)), int(m.groups()[-1]))
            msg = msg[:m.start()]
        else:
            m = re.search(r' while \\output is active', msg)
            if m:
                lineno = None
                msg = msg[:m.end()]
            else:
                self.__message('warning', None,
                               'malformed bad box message in log')
                return
        # Back up to the end of the known message text
        self.__pos = origpos + m.end()
        if self.__lookingat('\n'):
            # We have a newline, so consume it and look for the
            # offending text.
            self.__pos += 1
            # If there is offending text, it will start with a font
            # name, which will start with a \.
            if 'hbox' in msg and self.__lookingat('\\'):
                self.__consume_line(unwrap=True)
        msg = self.__simplify_message(msg) + ' (page {})'.format(self.__pageno)
        cls = msg.split(None, 1)[0].lower()
        self.__message('warning', lineno, msg, cls=cls)

    def __generic_warning(self):
        # Warnings produced by LaTeX's \GenericWarning (which is
        # called by \{Package,Class}Warning and \@latex@warning),
        # warnings produced by pdftex_warn, and other random warnings.
        msg, cls = self.__generic_info()
        # Most warnings include an input line emitted by \on@line
        m = re.search(' on input line ([0-9]+)', msg)
        if m:
            lineno = int(m.group(1))
            msg = msg[:m.start()]
        else:
            lineno = None
        msg = self.__simplify_message(msg)
        self.__message('warning', lineno, msg, cls=cls)

    def __generic_info(self):
        # Messages produced by LaTeX's \Generic{Error,Warning,Info}
        # and things that look like them
        msg = self.__consume_line(unwrap=True).strip()
        # Package and class messages are continued with lines
        # containing '(package name)            '
        pkg_name = msg.split(' ', 2)[1]
        prefix = '(' + pkg_name + ')            '
        while self.__lookingat(prefix):
            # Collect extra lines.  It's important that we keep these
            # because they may contain context information like line
            # numbers.
            extra = self.__consume_line(unwrap=True)
            msg += ' ' + extra[len(prefix):].strip()
        return msg, pkg_name.lower()

##################################################################
# BibTeX task
#

class BibTeX(Task):
    def __init__(self, db, latex_task, cmd, cmd_args, nowarns, obj_dir):
        super().__init__(db, 'bibtex::' + normalize_input_path(
            latex_task.get_tex_filename()))
        self.__latex_task = latex_task
        self.__cmd = cmd
        self.__cmd_args = cmd_args
        self.__obj_dir = obj_dir

    def stable(self):
        # If bibtex doesn't have its inputs, then it's stable because
        # it has no effect on system state.
        jobname = self.__latex_task.get_jobname()
        if jobname is None:
            # We don't know where the .aux file is until latex has run
            return True
        if not os.path.exists(jobname + '.aux'):
            # Input isn't ready, so bibtex will simply fail without
            # affecting system state.  Hence, this task is trivially
            # stable.
            return True
        if not self.__find_bib_cmds(os.path.dirname(jobname), jobname + '.aux'):
            # The tex file doesn't refer to any bibliographic data, so
            # don't run bibtex.
            return True

        return super().stable()

    def __find_bib_cmds(self, basedir, auxname, stack=()):
        debug('scanning for bib commands in {}'.format(auxname))
        if auxname in stack:
            raise TaskError('.aux file loop')
        stack = stack + (auxname,)

        try:
            aux_data = open(auxname, errors='surrogateescape').read()
        except FileNotFoundError:
            # The aux file may not exist if latex aborted
            return False
        if re.search(r'^\\bibstyle\{', aux_data, flags=re.M) or \
           re.search(r'^\\bibdata\{',  aux_data, flags=re.M):
            return True

        if re.search(r'^\\abx@aux@cite\{', aux_data, flags=re.M):
            # biber citation
            return True

        # Recurse into included aux files (see aux_input_command), in
        # case \bibliography appears in an \included file.
        for m in re.finditer(r'^\\@input\{([^}]*)\}', aux_data, flags=re.M):
            if self.__find_bib_cmds(basedir, os.path.join(basedir, m.group(1)),
                                    stack):
                return True

        return False

    def _input_args(self):
        if self.__is_biber():
            aux_name = os.path.basename(self.__latex_task.get_jobname())
        else:
            aux_name = os.path.basename(self.__latex_task.get_jobname()) + '.aux'
        return [self.__cmd] + self.__cmd_args + [aux_name]

    def _input_cwd(self):
        return os.path.dirname(self.__latex_task.get_jobname())

    def _input_auxfile(self, auxname):
        # We don't consider the .aux files regular inputs.
        # Instead, we extract just the bit that BibTeX cares about
        # and depend on that.  See get_aux_command_and_process in
        # bibtex.web.
        debug('hashing filtered aux file {}', auxname)
        try:
            with open(auxname, 'rb') as aux:
                h = hashlib.sha256()
                for line in aux:
                    if line.startswith((b'\\citation{', b'\\bibdata{',
                                        b'\\bibstyle{', b'\\@input{',
                                        b'\\abx@aux@cite{')):
                        h.update(line)
                return h.hexdigest()
        except FileNotFoundError:
            debug('{} does not exist', auxname)
            return None

    def __path_join(self, first, rest):
        if rest is None:
            # Append ':' to keep the default search path
            return first + ':'
        return first + ':' + rest

    def __is_biber(self):
        return "biber" in self.__cmd

    def _execute(self):
        # This gets complicated when \include is involved.  \include
        # switches to a different aux file and records its path in the
        # main aux file.  However, BibTeX does not consider this path
        # to be relative to the location of the main aux file, so we
        # have to run BibTeX *in the output directory* for it to
        # follow these includes (there's no way to tell BibTeX other
        # locations to search).  Unfortunately, this means BibTeX will
        # no longer be able to find local bib or bst files, but so we
        # tell it where to look by setting BIBINPUTS and BSTINPUTS
        # (luckily we can control this search).  We have to pass this
        # same environment down to Kpathsea when we resolve the paths
        # in BibTeX's log.
        args, cwd = self._input('args'), self._input('cwd')
        debug('running {} in {}', args, cwd)

        env = os.environ.copy()
        env['BIBINPUTS'] = self.__path_join(os.getcwd(), env.get('BIBINPUTS'))
        env['BSTINPUTS'] = self.__path_join(os.getcwd(), env.get('BSTINPUTS'))

        try:
            verbose_cmd(args, cwd, env)
            p = subprocess.Popen(args, cwd=cwd, env=env,
                                 stdin=subprocess.DEVNULL,
                                 stdout=subprocess.PIPE,
                                 stderr=subprocess.STDOUT)
            stdout = self.__feed_terminal(p.stdout)
            status = p.wait()
        except OSError as e:
            raise TaskError('failed to execute bibtex task: ' + str(e)) from e

        inputs, auxnames, outbase = self.__parse_inputs(stdout, cwd, env)
        if not inputs and not auxnames:
            # BibTeX failed catastrophically.
            print(stdout, file=sys.stderr)
            raise TaskError('failed to execute bibtex task')

        # Register environment variable inputs
        for env_var in ['TEXMFOUTPUT', 'BSTINPUTS', 'BIBINPUTS', 'PATH']:
            self._input('env', env_var)

        # Register file inputs
        for path in auxnames:
            self._input('auxfile', path)
        for path in inputs:
            self._input('file', path)

        if self.__is_biber():
            outbase = os.path.join(cwd, outbase)
        outputs = [outbase + '.bbl', outbase + '.blg']
        return RunResult(outputs, {'outbase': outbase, 'status': status,
                                   'inputs': inputs})

    def __feed_terminal(self, stdout):
        with Progress('bibtex') as progress:
            buf, linebuf = [], ''
            while True:
                data = os.read(stdout.fileno(), 4096)
                if not data:
                    break
                # See "A note about encoding" above
                data = data.decode('ascii', errors='surrogateescape')
                buf.append(data)
                linebuf += data
                while '\n' in linebuf:
                    line, _, linebuf = linebuf.partition('\n')
                    if line.startswith('Database file'):
                        progress.update(line.split(': ', 1)[1])
        return ''.join(buf)

    def __parse_inputs(self, log, cwd, env):
        # BibTeX conveniently logs every file that it opens, and its
        # log is actually sensible (see calls to a_open_in in
        # bibtex.web.)  The only trick is that these file names are
        # pre-kpathsea lookup and may be relative to the directory we
        # ran BibTeX in.
        #
        # Because BibTeX actually depends on very little in the .aux
        # file (and it's likely other things will change in the .aux
        # file), we don't count the whole .aux file as an input, but
        # instead depend only on the lines that matter to BibTeX.
        kpathsea = Kpathsea('bibtex')
        inputs = []
        auxnames = []
        outbase = None
        for line in log.splitlines():
            m = re.match('(?:The top-level auxiliary file:'
                         '|A level-[0-9]+ auxiliary file:) (.*)', line)
            if m:
                auxnames.append(os.path.join(cwd, m.group(1)))
                continue
            m = re.match('(?:(The style file:)|(Database file #[0-9]+:)) (.*)',
                         line)
            if m:
                filename = m.group(3)
                if m.group(1):
                    filename = kpathsea.find_file(filename, 'bst', cwd, env)
                elif m.group(2):
                    filename = kpathsea.find_file(filename, 'bib', cwd, env)

                # If this path is relative to the source directory,
                # clean it up for error reporting and portability of
                # the dependency DB
                if filename.startswith('/'):
                    relname = os.path.relpath(filename)
                    if '../' not in relname:
                        filename = relname

                inputs.append(filename)

            # biber output
            m = re.search("Found BibTeX data source '(.*?)'",
                         line)
            if m:
                filename = m.group(1)
                inputs.append(filename)

            m = re.search("Logfile is '(.*?)'", line)
            if m:
                outbase = m.group(1)[:-4]

        if outbase is None:
            outbase = auxnames[0][:-4]

        return inputs, auxnames, outbase

    def report(self):
        extra = self._get_result_extra()
        if extra is None:
            return 0

        # Parse and pretty-print the log
        log = open(extra['outbase'] + '.blg', 'rt').read()
        inputs = extra['inputs']
        for msg in BibTeXFilter(log, inputs).get_messages():
            msg.emit()

        # BibTeX exits with 1 if there are warnings, 2 if there are
        # errors, and 3 if there are fatal errors (sysdep.h).
        # Translate to a normal UNIX exit status.
        if extra['status'] >= 2:
            return 1
        return 0

class BibTeXFilter:
    def __init__(self, data, inputs):
        self.__inputs = inputs
        self.__key_locs = None

        self.__messages = []

        prev_line = ''
        for line in data.splitlines():
            msg = self.__process_line(prev_line, line)
            if msg is not None:
                self.__messages.append(Message(*msg))
            prev_line = line

    def get_messages(self):
        """Return a list of warning and error Messages."""
        # BibTeX reports most errors in no particular order.  Sort by
        # file and line.
        return sorted(self.__messages,
                      key=lambda msg: (msg.filename or '', msg.lineno or 0))

    def __process_line(self, prev_line, line):
        m = None
        def match(regexp):
            nonlocal m
            m = re.match(regexp, line)
            return m

        # BibTeX has many error paths, but luckily the set is closed,
        # so we can find all of them.  This first case is the
        # workhorse format.
        #
        # AUX errors: aux_err/aux_err_return/aux_err_print
        #
        # BST errors: bst_ln_num_print/bst_err/
        # bst_err_print_and_look_for_blank_line_return/
        # bst_warn_print/bst_warn/
        # skip_token/skip_token_print/
        # bst_ext_warn/bst_ext_warn_print/
        # bst_ex_warn/bst_ex_warn_print/
        # bst_mild_ex_warn/bst_mild_ex_warn_print/
        # bst_string_size_exceeded
        #
        # BIB errors: bib_ln_num_print/
        # bib_err_print/bib_err/
        # bib_warn_print/bib_warn/
        # bib_one_of_two_expected_err/macro_name_warning/
        if match('(.*?)---?line ([0-9]+) of file (.*)'):
            # Sometimes the real error is printed on the previous line
            if m.group(1) == 'while executing':
                # bst_ex_warn.  The real message is on the previous line
                text = prev_line
            else:
                text = m.group(1) or prev_line
            typ, msg = self.__canonicalize(text)
            return (typ, m.group(3), int(m.group(2)), msg)

        # overflow/print_overflow
        if match('Sorry---you\'ve exceeded BibTeX\'s (.*)'):
            return ('error', None, None, 'capacity exceeded: ' + m.group(1))
        # confusion/print_confusion
        if match('(.*)---this can\'t happen$'):
            return ('error', None, None, 'internal error: ' + m.group(1))
        # aux_end_err
        if match('I found (no .*)---while reading file (.*)'):
            return ('error', m.group(2), None, m.group(1))
        # bad_cross_reference_print/
        # nonexistent_cross_reference_error/
        # @<Complain about a nested cross reference@>
        #
        # This is split across two lines.  Match the second.
        if match('^refers to entry "'):
            typ, msg = self.__canonicalize(prev_line + ' ' + line)
            msg = re.sub('^a (bad cross reference)', '\\1', msg)
            # Try to give this key a location
            filename = lineno = None
            m2 = re.search(r'--entry "[^"]"', prev_line)
            if m2:
                filename, lineno = self.__find_key(m2.group(1))
            return (typ, filename, lineno, msg)
        # print_missing_entry
        if match('Warning--I didn\'t find a database entry for (".*")'):
            return ('warning', None, None,
                    'no database entry for ' + m.group(1))
        # x_warning
        if match('Warning--(.*)'):
            # Most formats give warnings about "something in <key>".
            # Try to match it up.
            filename = lineno = None
            for m2 in reversed(list(re.finditer(r' in ([^, \t\n]+)\b', line))):
                if m2:
                    filename, lineno = self.__find_key(m2.group(1))
                    if filename:
                        break
            return ('warning', filename, lineno, m.group(1))
        # @<Clean up and leave@>
        if match('Aborted at line ([0-9]+) of file (.*)'):
            return ('info', m.group(2), int(m.group(1)), 'aborted')

        # biber type errors
        if match('^.*> WARN - (.*)$'):
            print ('warning', None, None, m.group(1))
            m2 = re.match("(.*) in file '(.*?)', skipping ...", m.group(1))
            if m2:
                return ('warning', m2.group(2), "0", m2.group(1))
            return ('warning', None, None, m.group(1))

        if match('^.*> ERROR - (.*)$'):
            m2 = re.match("BibTeX subsystem: (.*?), line (\d+), (.*)$", m.group(1))
            if m2:
                return ('error', m2.group(1), m2.group(2), m2.group(3))
            return ('error', None, None, m.group(1))


    def __canonicalize(self, msg):
        if msg.startswith('Warning'):
            msg = re.sub('^Warning-*', '', msg)
            typ = 'warning'
        else:
            typ = 'error'
        msg = re.sub('^I(\'m| was)? ', '', msg)
        msg = msg[:1].lower() + msg[1:]
        return typ, msg

    def __find_key(self, key):
        if self.__key_locs is None:
            p = BibTeXKeyParser()
            self.__key_locs = {}
            for filename in self.__inputs:
                data = open(filename, 'rt', errors='surrogateescape').read()
                for pkey, lineno in p.parse(data):
                    self.__key_locs.setdefault(pkey, (filename, lineno))
        return self.__key_locs.get(key, (None, None))

class BibTeXKeyParser:
    """Just enough of a BibTeX parser to find keys."""

    def parse(self, data):
        IDENT_RE = '(?![0-9])([^\x00-\x20\x80-\xff \t"#%\'(),={}]+)'
        self.__pos, self.__data = 0, data
        # Find the next entry
        while self.__consume('[^@]*@[ \t\n]*'):
            # What type of entry?
            if not self.__consume(IDENT_RE + '[ \t\n]*'):
                continue
            typ = self.__m.group(1)
            if typ == 'comment':
                continue
            start = self.__pos
            if not self.__consume('([{(])[ \t\n]*'):
                continue
            closing, key_re = {'{' : ('}', '([^, \t\n}]*)'),
                               '(' : (')', '([^, \t\n]*)')}[self.__m.group(1)]
            if typ not in ('preamble', 'string'):
                # Regular entry; get key
                if self.__consume(key_re):
                    yield self.__m.group(1), self.__lineno()
            # Consume body of entry
            self.__pos = start
            self.__balanced(closing)

    def __consume(self, regexp):
        self.__m = re.compile(regexp).match(self.__data, self.__pos)
        if self.__m:
            self.__pos = self.__m.end()
        return self.__m

    def __lineno(self):
        return self.__data.count('\n', 0, self.__pos) + 1

    def __balanced(self, closing):
        self.__pos += 1
        level = 0
        skip = re.compile('[{}' + closing + ']')
        while True:
            m = skip.search(self.__data, self.__pos)
            if not m:
                break
            self.__pos = m.end()
            ch = m.group(0)
            if level == 0 and ch == closing:
                break
            elif ch == '{':
                level += 1
            elif ch == '}':
                level -= 1

class Kpathsea:
    def __init__(self, program_name):
        self.__progname = program_name

    def find_file(self, name, format, cwd=None, env=None):
        """Return the resolved path of 'name' or None."""

        args = ['kpsewhich', '-progname', self.__progname, '-format', format,
                name]
        try:
            verbose_cmd(args, cwd, env)
            path = subprocess.check_output(
                args, cwd=cwd, env=env, universal_newlines=True).strip()
        except subprocess.CalledProcessError as e:
            if e.returncode != 1:
                raise
            return None
        if cwd is None:
            return path
        return os.path.join(cwd, path)

if __name__ == "__main__":
    main()


==> bin/mkabstract <==
#!/usr/bin/env python3

import os
import sys
import re
import textwrap

if len(sys.argv) != 3:
    print("[usage] %s [p.tex] [abstract.tex]" % sys.argv[0])
    exit(0)

pn_main = sys.argv[1]
pn_abst = sys.argv[2]

def get_sys(tex):
    tok = re.findall(r"\\newcommand{\\sys}{\\mbox{\\textsc{([^}]*)}", tex)
    if len(tok) == 0:
        print("Failed to find 'sys'")
        exit(1)
    return tok[0]

SYS = get_sys(open(pn_main).read())

abstract = []
for l in open(pn_abst):
    l = l.strip()
    if l.startswith("%"):
        continue
    if "{abstract}" in l:
        continue
    l = l.replace("\\%", "%")
    l = l.replace("\\emph{", "")
    l = l.replace("{", "")
    l = l.replace("}", "")
    l = l.replace("~", " ")
    l = l.replace("\\,", " ")
    l = l.replace("\\X", "x")
    l = l.replace("---", " -- ")
    l = l.replace("--", "-")
    l = l.replace("\\sys", SYS)
    l = l.replace("\\ie", "i.e.")
    l = l.replace("\\eg", "e.g.")
    l = l.replace("\\etal", " et al.")
    l = l.replace("\\Bs", " B/s")
    l = l.replace("\\KBs", " KB/s")
    l = l.replace("\\MBs", " MB/s")
    l = l.replace("\\GBs", " GB/s")
    l = l.replace("\\KB", " KB")
    l = l.replace("\\MB", " MB")
    l = l.replace("\\GB", " GB")
    l = l.replace("\\TB", " TB")
    l = l.replace("\\B", " B")
    l = l.replace("\\K", " K")
    l = l.replace("\\M", " M")
    l = l.replace("\\T", " T")
    
    if "\\" in l:
        print("WARN: unresolved char in")
        print(" > %s" % l)
        exit(1)

    abstract.append(l)

print("\n".join(abstract))


==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/fp.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cm}{/*}\PY{c+cm}{ Old version }\PY{c+cm}{*/}
\PY{k}{Result}\PY{+w}{  }\PY{p}{(}\PY{n}{estimated}\PY{o}{=}\PY{l+m+mi}{505284}\PY{p}{)}\PY{+w}{ }\PY{p}{(}\PY{n}{actual}\PY{o}{=}\PY{l+m+mi}{0}\PY{p}{)}
\PY{+w}{ }\PY{n}{One}\PY{o}{\PYZhy{}}\PY{n+nc}{Time}\PY{+w}{ }\PY{k}{Filter}\PY{+w}{ }\PY{p}{(}\PY{n}{pg\PYZus{}stat\PYZus{}get\PYZus{}snapshot\PYZus{}timestamp}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{now}\PY{p}{(}\PY{p}{)}\PY{p}{)}
\PY{+w}{ }\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{Hash}\PY{+w}{ }\PY{k}{Join}\PY{+w}{ }\PY{p}{(}\PY{n}{estimated}\PY{o}{=}\PY{l+m+mi}{505284}\PY{p}{)}\PY{p}{(}\PY{n}{never}\PY{+w}{ }\PY{n}{executed}\PY{p}{)}
\PY{+w}{  }\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{+w}{  }\PY{n}{Seq}\PY{+w}{ }\PY{n}{Scan}\PY{+w}{ }\PY{k}{on}\PY{+w}{ }\PY{n}{stock}\PY{+w}{ }\PY{n}{ref\PYZus{}0}\PY{+w}{ }\PY{p}{(}\PY{n}{estimated}\PY{o}{=}\PY{l+m+mi}{505284}\PY{p}{)}\PY{p}{(}\PY{n}{never}\PY{+w}{ }\PY{n}{executed}\PY{p}{)}

\PY{c+cm}{/*}\PY{c+cm}{ New version }\PY{c+cm}{*/}
\PY{k}{Result}\PY{+w}{  }\PY{p}{(}\PY{n}{estimated}\PY{o}{=}\PY{l+m+mi}{100000}\PY{p}{)}\PY{+w}{ }\PY{p}{(}\PY{n}{actual}\PY{o}{=}\PY{l+m+mi}{100000}\PY{+w}{ }\PY{n}{loops}\PY{o}{=}\PY{l+m+mi}{1}\PY{p}{)}
\PY{+w}{ }\PY{n}{One}\PY{o}{\PYZhy{}}\PY{n+nc}{Time}\PY{+w}{ }\PY{k}{Filter}\PY{+w}{ }\PY{p}{(}\PY{n}{pg\PYZus{}stat\PYZus{}get\PYZus{}snapshot\PYZus{}timestamp}\PY{p}{(}\PY{p}{)}\PY{+w}{ }\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{now}\PY{p}{(}\PY{p}{)}\PY{p}{)}
\PY{+w}{ }\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{Hash}\PY{+w}{ }\PY{k}{Join}\PY{+w}{ }\PY{p}{(}\PY{n}{estimated}\PY{o}{=}\PY{l+m+mi}{100000}\PY{p}{)}\PY{+w}{ }\PY{p}{(}\PY{n}{actual}\PY{o}{=}\PY{l+m+mi}{100000}\PY{p}{)}
\PY{+w}{  }\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{+w}{ }\PY{n}{Seq}\PY{+w}{ }\PY{n}{Scan}\PY{+w}{ }\PY{k}{on}\PY{+w}{ }\PY{n}{stock}\PY{+w}{ }\PY{n}{ref\PYZus{}0}\PY{+w}{ }\PY{p}{(}\PY{n}{estimated}\PY{o}{=}\PY{l+m+mi}{100000}\PY{p}{)}\PY{+w}{ }\PY{p}{(}\PY{n}{actual}\PY{o}{=}\PY{l+m+mi}{100000}\PY{p}{)}
\end{Verbatim}


==> code/patch1.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{switch}\PY{p}{(} \PY{n}{pExpr}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{op} \PY{p}{)}\PY{p}{\PYZob{}}
    \PY{p}{.}\PY{p}{.}\PY{p}{.}
    \PY{k}{case} \PY{n+nl}{TK\PYZus{}ISNULL}\PY{p}{:}
    \PY{k}{case} \PY{n+nl}{TK\PYZus{}NOTNULL}\PY{p}{:} \PY{c+c1}{//ADDED: IS NOT NULL case}
    \PY{k}{case} \PY{n+nl}{TK\PYZus{}FUNCTION}\PY{p}{:}
      \PY{c+c1}{// Omit children but continue walking siblings}
      \PY{k}{return} \PY{n}{WRC\PYZus{}Prune}\PY{p}{;}
    \PY{k}{default}\PY{o}{:}
      \PY{c+c1}{// Continue down into children }
      \PY{k}{return} \PY{n}{WRC\PYZus{}Continue}\PY{p}{;}
\end{Verbatim}


==> driftdetectionalgos.tex <==
\PP{Types of Drift Detection Algorithms}
% 
We categorize drift detection algorithms based on whether they require
labels or not (\ie, an oracle's feedback): 
(1) supervised~\cite{drift2}, or (2) unsupervised techniques \cite{md3b}.
%
In this paper, we restrict our focus to unsupervised techniques since 
\sys must function even in the absence of an oracle's feedback.
%
Prior techniques for unsupervised drift detection in \textit{closed-world}
\footnote{In a closed-world dataset, the set of target classes is fixed at 
training time. In contrast, in an open-world dataset, the set of target classes
may evolve at testing time.} datasets include:





\squishitemize
\item \textbf{Model Confidence Methods}: 
%
These methods~\cite{trustclass,md3b} do not generalize to visual data with drift.
%
Their distance metric is defined in terms of the model's decision boundary.
%
So, with drift, the raw distance scores require re-calibration~\cite{confidence1}.
%
If the confidence scores are not properly calibrated, the resulting overly
confident models will incorrectly judge their own 
performance~\cite{confidence2,trustclass}.
%

\item \textbf{Clustering Algorithms}: 
%
These algorithms also do not generalize to visual data with
drift~\cite{olindda,samknn}.
%
This is because widely used distance metrics (\eg, $L_2$ norm) do not work well 
with high-dimensional data due to the curse of dimensionality.
%
For instance, with the $L_2$ norm, the volume of the unit hypersphere approaches
zero\footnote{$Volume(d)=0.5^d\pi^{0.5d}/\Gamma(0.5d + 1)$, 
where d represents the number of dimensions.}, most points exist at the corners
of the unit hypercube, rendering the metric ineffective.
\squishend



==> response.tex <==
%\documentclass{article}
%\usepackage{booktabs}
%\usepackage{xcolor}
%\usepackage{endnotes,microtype,xspace,graphicx,fancyvrb,multirow}
%\usepackage{cleveref}

%\begin{document}
\section*{Revision Response}

We would like to thank all of the reviewers for their helpful critiques and
questions. The revised version of this paper represents a substantial effort
on our part to expand our experimental evaluation and improve our presentation
based on the feedback. We made the following revisions:

\squishitemize
\item We conducted a set of additional experiments including: 
\squishitemize
\item Query experiment focusing on visual DBMS tasks 
\item Model generation and query execution time analysis 
\item Ablation study to delineate the impact of different components of \sys.
\squishend
%
\item We highlight the connection between \sys and other visual DBMSs to
clarify its relevance to the database community in~\autoref{sec:eval:queries}.
%
\item We revised the paper to improve its readability and clarity based on the
feedback from the reviewers.
\squishend

We believe that these changes improve the technical and research contributions
of the paper. We have highlighted all of the changes made in the body of the
paper.
\\

%% ==================================================================
%% Meta-Reviewer
%% ==================================================================

\separator
\section*{Response to Meta-Reviewer}

\response{1}{The relevance to DB community is unclear. Efficiency issues, 
including models generation times and processing execution times should be 
discussed and reported.}

We thank the reviewers for highlighting these issues.
%
Based on the feedback from the reviewers, we conducted these additional 
experiments to examine the efficiency issues and to clarify the relevance to the
DB community~\cite{blazeit,videoedge,deeplens,chameleon}:

\squishitemize

\item 
\PP{Aggregation Query} 
We measure the query accuracy of \sys compared to a static system. We use
an aggregation query that count the number of a specific class in \bdd (\eg a query
to count the number of `cars'), and show results for four 
classes in~\autoref{sec:eval:queries}.
%
Our aggregation query experiment shows that \sys delivers higher detection accuracy with 
higher throughput compared to a static approach. The cross-subset accuracy in ~\autoref{tab:performances}
better explains this discrepancy: \sys performs well across the board on \daydata,
\nightdata, \rainydata, and \snowydata. 
%
In contrast, a static approach has poor detection accuracy
across dataset subsets. Consequently, the query accuracy also suffers.

\item 
\PP{Model Generation Time} 
%
We compare the time taken to generate models within \sys against a canonical
visual DBMS without drift recovery in~\autoref{sec:eval::specialization}.
%
On \nightdata, \sys generates a \yololocal model 21$\times$ faster compared
to an off-the-shelf unspecialized \yolo model.
%
The reasons for this are twofold.
%
First, the specialized model consists of 7$\times$ fewer parameters compared to
the original \yolo model.
%
Second, the \nightdata cluster contains 3$\times$ fewer images compared to
\fulldata.
%
Reduction in model and dataset sizes leads to faster training of specialized
models. 

\item 
\textbf{Query Execution Time:} 
%
We next compare the time taken to execute queries with and without drift 
recovery in~\autoref{sec:eval::specialization}.
%
\sys{'s} \yololocal model is 6$\times$ faster than the \yolo model used in
state-of-the-art visual DBMSs~\cite{blazeit,chameleon}.
%
This is because of it consists of fewer convolution operations.

\item
\PP{Accuracy} 
%
We have compared the accuracy of \yolo and \yololocal models in ~\autoref{fig:locallite}. 
%
On \nightdata, the \yololocal model delivers 2$\times$ higher accuracy.
%
Furthermore, it improves accuracy by 1.5$\times$ on average across all clusters.
%

Thus, specialized models enable faster and more accurate query processing over
visual data.

\item 
\PP{Ablation Study} 
%
We have also added an ablation study in ~\autoref{sec:eval:ablation}. Here, we examine the impact
of each of \sys{'s} components by removing them and comparing detection and query accuracy. 
%
We show results of removing  \selector, \detector, and \specializer on detection and query accuracy in 
~\autoref{tab:ablation}.
%
Removing \selector reduces detection accuracy by almost 40\%, from 40 mAP to 24 mAP.
%
Query accuracy is reduced by nearly 25\%.
%
Further removing the \detector and \specializer and replacing \sys with a static system reduces detection accuracy 
by a further 15\%, from 24 mAP to 20 mAP.
%
Query accuracy is reduced by 10\%. 
\squishend

\response{2}{The difference between drift detection and recovery and domain 
adaptation needs to be discussed.}

We thank the meta-reviewer for this suggestion.
%
Domain adaptation consists of learning in a non-stationary environment, in which
the underlying data distribution (\ie, the joint distribution of the input data
and labels P(X,Y)) evolves over time.
%
Domain adaptation is also referred to as \textit{concept drift} in the
literature~\cite{drift2,drift3}.
%
We classify the changes in the data distribution into two categories:
(1) real drift (\aka, task drift), and (2) virtual drift (\aka, domain drift) \cite{bengio}.
%
The key distinction between virtual and real drift is that the \textit{real}
decision boundary only changes under real drift.
%

Real drift reflects real changes in the world and is exemplified by changes in
fashion (\eg, modern music).
%
Formally, this corresponds to the drift  in the conditional distribution of
labels given the input data (\ie, P(Y | X)), often resulting from an updated
definition of the task necessitating a change in the predictive function from
the input space to label space.
%
So, this is also referred to as task drift.

Virtual drift does not occur in reality but rather occurs in the
deep learning model reflecting this reality.
%
In practice, this type of drift arises when the model does not identify all the
relevant features or cannot cope with class imbalance.
%
Formally,  this corresponds to the drift in the marginal distribution of the
input data (\ie, P(X)), with an additional assumption that P(Y | X) remains the
same.
%
So, this is also referred to as domain drift.

\sys only copes with virtual drift.
%
\detector measures changes in the marginal distribution of the input data (\ie,
P(X)).
%
\sys recovers from drift using: (1) unsupervised (\ie, \yololite model), and (2)
supervised domain adaptation (\ie, \yololocal model) algorithms.
%
As shown in~\autoref{fig:locallite}, the \yololite model learned via
unsupervised domain adaptation delivers lower accuracy compared to the
\yololocal model learned in a supervised setting.
%
The \yololocal model delivers 1.5--2$\times$ higher accuracy compared to the
original \yolo model across all clusters.
%
In contrast, \yololite only performs slightly better than the \yolo model 
on \daydata, \rainydata, and \snowydata clusters, and delivers lower accuracy on
\nightdata.
%
In general, unsupervised domain adaptation is active area of research.
%
We plan to investigate how to improve the efficacy of unsupervised domain
adaptation for drift recovery in the future.

\response{3}{The experimental part needs to be strengthened through 
comparisons with the state-of-the-arts and a more suitable design for ablation study.}

Based on the reviewers' feedback, in addition to the experiments covered in our
response to \textbf{MR.1}, we conducted these experiments:

\squishitemize
\item \PP{Efficacy of Drift Detector:}
%
We compared the efficacy of DA-GAN in detecting drift against that of PCA on the
MNIST dataset. 
%
The results are summarized in ~\autoref{tab:mnistperf}.

\item \PP{Ablation Study:}
%
We conducted an ablation study to delineate the impact of the drift detection,
recovery, and model selection components of \sys in~\autoref{sec:eval:ablation}.
%
Since the \detector is not useful without the recovery components, we consider
these configurations:
%
\squishitemize
\item End-to-End System: With all three components.
\item - \selector: With only the \detector and \specializer components.
%
\sys uses the most recently created \yololocal model in this setting.
%
%\item Impact of \detector: Next, we remove the drift detection module
%\footnote{We cannot remove \specializer first, because  that would  leave 
%\sys with only a \detector, which would then not be used}, and leave 
%\specializer. 
%
%Since \specializer  depends on \detector to generate models, we tweak it as
%follows: \sys is initialized with specialized models for all clusters, an
%ensemble of specialized models is used for evaluation.
%
\item Baseline: Lastly, we remove all the three components.
%
In this configuration, \sys uses the heavyweight \yolo model.
%
\squishend
\squishend

We summarize the results in~\autoref{tab:ablation}. 
%
Eliminating the \selector leads to a drop in accuracy, since the best model is
no longer used for each cluster. 
%
The naive model selection policy is only useful when the drift is monotonically
increasing.
%
In practice, older clusters co-exist with newer clusters, as is the case in
\bdd.
%
Since the most recent model is trained on newer clusters, its accuracy drops
when older clusters are re-introduced.
%
%Detection accuracy falls by nearly 40\%, and query accuracy falls by 25\%. 
%
The memory footprint and throughput are nearly unchanged, since the \selector is
computationally lightweight.
%
Lastly, removing the \detector and \specializer is equivalent to using a static
heavyweight \yolo model.
%
The lack of specialization leads to lower accuracy.
%
Furthermore, performance also suffers since the \yolo model is larger and slower
than the \yololocal models constructed by the \specializer.



\begin{figure}[t]
	\centering
	\hfill	
	\begin{subfigure}{.4\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figs/aelatent}
		\caption{Standard Autoencoder}
		\label{fig:responseaelatent}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.4\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figs/vaelatent}
		\caption{Variational Autoencoder}
		\label{fig:responsevaelatent}
	\end{subfigure}
	\hfill
	\\
	\hfill	
	\begin{subfigure}{.4\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figs/aaelatent}
		\caption{Adversarial Autoencoder}
		\label{fig:responseaaelatent}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.4\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figs/daganlatent}
		\caption{DA-GAN}
		\label{fig:responsedaganlatent}
	\end{subfigure}
	\hfill
	
	\caption{\textbf{Latent Spaces}: 
	%
	The latent spaces associated with the autoencoders we considered in \sys.
	%
	Each sub-image in this grid is a point drawn uniformly from the 
	unit square ($[0,0]$ to $[1,1]$) and passed through the decoder. 
	%
	Blurry reconstruction indicates loss of information.}
	\label{fig:responselatents}
\end{figure}

\response{4}{It may be not correct to claim that "real drift always requires oracle 
supervision" (section 2.2). A number of unsupervised domain adaption algorithms 
have been proposed to tackle this issue.}

We concur with the reviewer that this statement is only partially correct. 
%
We could use weak-supervision techniques (\eg, Snorkel~\cite{snorkel}) to
generate labels for training models.
%
We have added this clarification in~\autoref{sec:preliminaries::drift}
and~\autoref{sec:discussionlimitation}.

\response{5}{Section 4.3: A justification is required for forcing the latent
vector z to approximate a normal distribution N(0,1).   
It is more reasonable and common to use variational autoencoder instead.
}

We considered using a variational autoencoder (AE).
%
As shown in ~\autoref{fig:responselatents}, the variational AE causes more 
blurriness than an adversarial AE after dimensionality reduction, 
thereby leading to a loss of information.
%
This is detrimental to \sys{'s} drift detection algorithm, since key
information about the distribution is lost.
%
In contrast, an adversarial AE performs better by reducing the blurriness and
preserving more information during dimensionality reduction~\cite{aae}.
%
So, we adopted this approach in \sys and combined it with a GAN to create the
DA-GAN architecture.
%; all architectures are summarized in ~\autoref{fig:architectures}.

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.9\textwidth]{figs/responseaes}
%	\caption{\textbf{Autoencoders and latent spaces}: 
%	The standard autoencoder (AE) has holes in the latent space due to irregular mapping.
%	%
%	The variational AE smoothes out the holes, but the smoothing process creates blurriness. This indicates
%	poor compression, or higher information loss. For drift detection, we would like a compressed
%	representation of the distribution that captures as much information as possible.
%	%
%	The adversarial AE removes holes and preserves enough distribution information for crisper reconstruction. So,
%	it is more effective for drift detection.}
%	\label{fig:responseaes}
%\end{figure}


\response{6}{Some definitions could be further polished. For example, regarding the 
definition of Virtual Drift, the data distribution change seems not to affect the 
classifier. In this case, why a model with new data or training a new model on the 
new distribution is required?}

Based on the reviewer's feedback, we have added formal definitions for 
different types of concept drift, as discussed in our response to \textbf{MR.2}.
%
We have added this clarification in~\autoref{sec:preliminaries::drift}.

We would like to clarify that the deep learning model learns a \textit{virtual}
decision boundary that is only an approximation of the \textit{real} decision
boundary. 
%
With virtual drift, even if the real decision boundary does not change, we need
to update the virtual decision boundary learned by the model to avoid a drop in
accuracy.
%
This allows the model to work well on newly observed clusters (\eg, a model
trained \daydata operating on newly observed \nightdata in \bdd).

\response{7}{In Equation 3, How to define $D_{KL} \rightarrow 0$ ?}

We thank the reviewer for raising this issue.
%
$D_{KL}\rightarrow 0$ when $P_B$ $=$ $P_A$.
%
Here, $\log(P_B(x)/P_A(x))$ $=$ $log(1)$ $=$ $0$.
%
This indicates lack of divergence between $P_B$ and $P_A$.
%
We added this clarification in~\autoref{sec:driftdetection::bands}.


%% ==================================================================
%% REVIEWER 1
%% ==================================================================

\separator
\reviewer{1}

\response{W1, W2}{
\textbf{End-to-End Analysis:}
The goals could be described and  verified with experiments in
a more succinct way. Why it is necessary to measure the 
efficacy of each part of the system (drift detection, model specialization 
and model selection) is not clear, provided that the ultimate goal is to
maximize the accuracy of object detection task.}

Based on the reviewer's feedback, we now place more emphasis on the end-to-end
accuracy of \sys on the given task.
%
Since it is harder to explain the empirical setup of the end-to-end experiment
in~\autoref{sec:eval::full} without describing the clusters identified by \sys
in \bdd, we present it at the end of the evaluation section.
% 
We added this clarification in~\autoref{sec:evaluation}.

We conducted a new experiment wherein we compare the \textit{query accuracy}
of \sys compared to a static setting without drift detection and recovery.
%
We summarize the results of this experiment in~\autoref{sec:eval:queries}.

Besides these end-to-end experiments, we studied the efficacy of each component
of the system to separately quantify the impact of our techniques.
%
Based on the reviewers' feedback, we have added an ablation study to delineate
the impact of the different components of \sys
in~\autoref{sec:eval:ablation}~\cite{ablation}. 
%

\response{D1}{
\textbf{Component-wise Analysis:}
\textbf{(1)}
While the drift detection result is good, it is not clear whether comparing with
mechanisms like LOF, AE, DRAE etc. was enough. 
Are these the most commonly used methods for drift detection in video
analytics? 
\textbf{(2)}
It was said that some clustering algorithms do not work well on high 
dimensional image data because of using l2 norm. Some of those clustering
methods could be tried out and their results could be shown.
}

\textbf{(1)}
%
LOF, AE, and DRAE are the state-of-the-art techniques for drift detection in
small-sized images~\cite{lof,drae,aae}.
%
Since they have been evaluated on \mnist and \cifar, we compare DA-GAN against
them on these datasets. 
%

\textbf{(2)}
%
We conducted a new experiment based on the reviewer's suggestion.
%
We compare DA-GAN against PCA~\cite{zou2006sparse} on drift detection.
%
We summarize these results in ~\autoref{tab:mnistperf}.

PCA does not work well on images due to their higher dimensionality.
%
This is because it performs linear dimensionality reduction and does not take
the spatial locality of the pixels in the image into consideration.
%
In contrast, LOF and DRAE work well on \mnist with fewer outliers.
%
However, their accuracy drops when they need to cope with more outliers. 
%
DA-GAN works well even when the percentage of outliers is high.
%
More importantly, it generalizes to larger-sized images, unlike AE and AAE.
%
This is critical for a video analytics system processing high-resolution
images.

We have added these results in~\autoref{sec:eval::detection}.

\response{D2}{\textbf{Benefits:} There is no benefit of drift 
detection unless a good mechanism can be established to recover 
from the drift. It is not clear why the paper had to show the 
results for each part of the system while there is a single 
ultimate goal. It appeared that the paper wants to detect objects 
in previously unseen environments. There are ten classes of objects 
(e.g., traffic lights, cars) and several environments (e.g., rainy, 
snowy, day, light etc.) in BDD dataset. Thus, an experiment could be 
designed where the system is trained on a subset of environments and 
then given the task of labeling the objects in novel environments. A 
section describing the results of this experiment would be enough to 
justify the effectiveness of the system. But it is not clear what 
information the result section conveys to the reader. Also, the accuracies 
provided in Table 4 and 5 are not usable, although better compared to 
the baselines.
}

We would like to clarify that the experiment in~\autoref{sec:eval::full} follows
the reviewer's suggestion.
%
However, we might not have placed enough emphasis on this end-to-end evaluation
of \sys on the given task.
%
We added this clarification in~\autoref{sec:eval::setup}.

We use the \bdd dataset to validate the efficacy of \sys across drifting
environmental conditions.
%
We initially train models on a subset of the \bdd dataset (\eg, \daydata).
%
We then introduce unseen clusters in \bdd during our evaluation (\eg,
\nightdata, \rainydata, and \snowydata) to examine
\sys{'s} drift detection and recovery capabilities.
%
When \detector detects drift due to the novelty of unseen clusters, 
the \specializer starts generating new models for these subsets and the
\selector picks them once they are generated.


As we discussed in our response to \textbf{R1.W1}, we conducted a new experiment
wherein we compare the \textit{query accuracy} of \sys compared to a static
setting without drift detection and recovery.
%
We summarize the results of this experiment with aggregation and filter queries 
in~\autoref{sec:eval:queries}.

\response{D3}{\textbf{Jargon:} As mentioned earlier, the 
paper is written with care, but the actual goals of the paper
 and how they were achieved could be presented more succinctly. 
 Rather than going through the deep-learning jargons and theories 
 from the very beginning, the overall process could be described in 
 terms of generic clustering and distancing concepts.
}

We thank the reviewer for this suggestion.
%
We have trimmed the sections on concept drift and generative models
in~\autoref{sec:motivation}.
%
We place more emphasis on the overall approach and used the reclaimed space to
present the results of the newly added experiments.

\response{D4}{
\textbf{(1)} \textbf{Motivating Example:} 
In motivating  example, the reader expects an example of the real-world scenario 
when the problem appears and why the problem persists due to the 
limitation of the existing system. But instead of describing that 
the paper shows some performance comparisons for the proposed system 
as motivating example. \\
%
\textbf{(2)} \textbf{Concept Drift Equation:} 
Also, the equation provided in Section 2.2 to 
clarify the definition of concept drift seems incorrect 
$$x^j=\sum_{i=1}^{N} w_{i}^j f_{i}^j$$. 
This equation and the associated description don't make any sense.
}

\PP{Motivating example}
%
Based on the reviewer's feedback, we now show a real-world illustration of drift
detection and recovery.
%
Specifically, we illustrate how a model trained on \rainydata, a cluster in
\bdd containing videos from overcast and rainy days, performs on \daydata,
another cluster in \bdd containing videos from clear, sunny days.
%
These two cluster are starkly different videos.
%
On \rainydata, the model needs to cope with occlusion caused by raindrops.
%
In contrast, \daydata contains bright reflections that make it difficult to
detect vehicles with lighter colors.

We compare \sys against a static system with drift detection and recovery
disabled.
%
We measure the detection accuracy and query accuracy metrics on these two
subsets.
%
Here, detection accuracy is the accuracy of the object detection model, and
query accuracy is the accuracy of the results of an aggregate query against the
ground truth.
%
We added the results of this motivating example
in~\autoref{sec:motivation::example}.

\PP{Equation}
%
We have updated our overview of concept drift
in~\autoref{sec:preliminaries::drift}.
%
We no longer present this equation in the paper.
%
However, we provide a clarification below.

$x=\sum_{i=1}^{N} w_{i} f_{i}$ represents a linear ML model (\eg linear
regressor), and an approximation of a non-linear ML model (\eg, neural
networks).
%
An ML model learns the appropriate weights for a given feature
matrix $f$ such that the predicted labels match the actual labels.
%
So, $w$ is an approximation of the true weight matrix $w^*$ that we are trying
to learn. 
%
With concept drift, $w^*$ evolves over time, rendering the $w$ that we have
learned inaccurate.
%
We incorporate this temporal change with the variable $j$ in the equation:

$$x^j=\sum_{i=1}^{N} w_{i}^j f_{i}^j$$


\response{D5}{\textbf{Metrics:} Since, the YOLO-specialized model was trained 
targeting specific clusters and not the whole data, the throughput and mem...}

We are not sure about this comment from the reviewer.
%
We would like to clarify that the memory footprint presented
in~\autoref{tab:yolostats} is that of the model (not the dataset).
%
Since we load the dataset in a batched manner, the model's throughput is
independent of the size of the dataset, and is only dependent on the model's
complexity.
%
Since \yololocal and \yololite are smaller than \yolo, they deliver higher
throughput on any dataset.


%% ==================================================================
%% REVIEWER 2
%% ==================================================================

\separator
\reviewer{2}

\response{W1}{\textbf{Recovery:} Although I found the provided experimental 
analysis extensive and convincing from an effectiveness point of view, with 
respect to efficiency, instead, I was wondering if it is possible to provides 
models generation times, and processing execution times. My comment is in line 
also with the discussions provided by the authors in the final "Limitations" Section.
}

We thank the reviewer for this suggestion.
%
We have added two experiments in~\autoref{sec:eval::specialization}. 

\squishitemize

\item 
\PP{Model Generation Time} 
%
We compare the time taken to generate models within \sys against a canonical
visual DBMS without drift recovery.
%
On \nightdata, \sys generates a \yololocal model 21$\times$ faster compared
to an off-the-shelf unspecialized \yolo model.
%
The reasons for this are twofold.
%
First, the specialized model consists of 7$\times$ fewer parameters compared to
the original \yolo model.
%
Second, the \nightdata cluster contains 3$\times$ fewer images compared to
\fulldata.
%
Reduction in model and dataset sizes leads to faster training of specialized
models. 

\item 
\textbf{Query Execution Time:} 
%
We next compare the time taken to execute queries with and without drift 
recovery in~\autoref{sec:eval::specialization}.
%
\sys{'s} \yololocal model is 6$\times$ faster than the \yolo model used in
state-of-the-art visual DBMSs~\cite{blazeit,chameleon}.
%
This is because of it consists of fewer convolution operations.

\squishend


%% ==================================================================
%% REVIEWER 3
%% ==================================================================

\separator
\reviewer{3}

\response{W1}{\textbf{Relevance:} The paper claims their system is a visual
DBMS, but the focus is on drift detection and recovery. I doubt the VLDB community 
is the right fit for the work.}

We concur with reviewer that drift detection and recovery is only a component of
a visual DBMS.
%
However, it complements the recent efforts taken by the database community in
designing visual DBMSs~\cite{blazeit,pp,chameleon,deeplens}.
%
The authors of BlazeIt~\cite{blazeit} mention that drift detection and recovery
is an important problem in practice.
%
Chameleon~\cite{chameleon}, another visual DBMS, adopts a manual approach to
constructing models specialized for diverse traffic conditions.
% 
By automatically detecting and recovering from drift, \sys delivers higher
accuracy even in the presence of drift.

To clarify the relevance to the state-of-the-art visual DBMSs, we added a new
experiment wherein we integrate and extend support for lightweight
filters and execute end-to-end queries~\cite{pp,blazeit}.
%
We present the results of this experiment in~\autoref{sec:eval:queries}.

\response{W2}{\textbf{End-to-End Experiments:} The experimental study is not
thorough and convincing.
There is only one end-to-end study on video analytics.}

We conducted additional experiments to strengthen our empirical analysis.
%
As discussed in \textbf{MR.1}, these experiments include:

\squishitemize

\item 
\PP{Aggregation Query} 
We measure the query accuracy of \sys compared to a static system. 
%
We focus on an aggregation query.
%
We also illustrate how \sys complements recent efforts in visual DBMSs by
integrating lightweight filters~\cite{pp,blazeit}.
%
As illustrated in~\autoref{fig:newarchitectures}, we consider three
configurations: 
(1) \sys with specialized models and no filters, 
(2) \syspp with specialized models and unspecialized filter~\cite{pp},  and 
(3) \sysfilter with specialized models and specialized filters. 
%
We present the results of these experiments in~\autoref{sec:eval:queries}.

\begin{figure}[t]
	\centering
	\begin{subfigure}{.85\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figs/odinbasic}
		\caption{\sys}
		\label{fig:odinbasicresponse}
	\end{subfigure}
	\\
	\begin{subfigure}{.95\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figs/odinppbasic}
		\caption{\syspp}
		\label{fig:odinppbasicresponse}
	\end{subfigure}
	\\
	\begin{subfigure}{.95\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figs/odinpp}
		\caption{\sysfilter}
		\label{fig:odinppresponse}
	\end{subfigure}
	\caption{\textbf{\sys Configurations}: 
	%
	We consider three configurations of \sys for evaluating an aggregation query. 
	%
	We defer a detailed description of these configurations
	to~\autoref{sec:eval:queries}.}
	\label{fig:newarchitectures}
\end{figure}


\item 
\PP{Model Generation Time} 
%
We compare the time taken to generate models within \sys against a canonical
visual DBMS without drift recovery in~\autoref{sec:eval::specialization}.


\item 
\textbf{Query Execution Time:} 
%
We next compare the time taken to execute queries with and without drift 
recovery in~\autoref{sec:eval::specialization}.
%
\sys{'s} \yololocal model is 6$\times$ faster than the \yolo model used in
state-of-the-art visual DBMSs~\cite{blazeit,chameleon}.

\item
\PP{Accuracy} 
%
We have compared the accuracy of \yolo and \yololocal models in ~\autoref{fig:locallite}. 
%
The specialized models in \sys enable faster and more accurate query processing over
visual data.

\item 
\PP{Ablation Study} 
%
We have added an ablation study in ~\autoref{sec:eval:ablation}. 
%
Here, we examine the impact of each of component of \sys by removing them and
comparing accuracy.
%
\squishend

\response{W3}{\textbf{Insights:} There is a lack of discussion of the insights
and key ideas of the proposed approach and the technical contribution is not very clear.}

%
\sys contains three components for tackling concept drift: 
drift detection, model specialization, and model selection.
%
We show that prior techniques for detecting drift do not work well on large
images~\cite{lof,drae}.
%
Since autoencoders are effective at image compression and GANs are effective at 
image generation, we combine these two networks to construct DA-GAN. 
%
The \detector uses the DA-GAN to learn the latent space of the images so that
it can identify previously unseen images.
%
This allows \sys to work well on large ($1280\times 720$), colored images in
\bdd.

We added this clarification in~\autoref{sec:eval::detection}.


\response{D1}{\textbf{Real System:} It is unclear if the system is a real
system or simply a theoretical/demo system.}

We would like to clarify that \sys is an end-to-end visual DBMS.
%
It is implemented in Python 3.6 and PyTorch 1.4
(\autoref{sec:eval::setup:::implementation}).
%
\sys supports aggregation queries using specialized models and
filters~\cite{blazeit,pp}.
%
We plan to add support for more complex queries in the future.

\separator

%
% Need to reset counter so paper sections start at 1
%
\setcounter{section}{0}



==> rev.tex <==
\gdef\therev{286633d}
\gdef\thedate{2020-07-21 12:58:21 -0700}

